Video Event Extraction via Tracking Visual States of Arguments

Video event extraction aims to detect salient events from a video and identify the arguments for each event as well as their semantic roles. Existing methods focus on capturing the overall visual scene of each frame, ignoring fine-grained argument-level information. Inspired by the definition of events as changes of states, we propose a novel framework to detect video events by tracking the changes in the visual states of all involved arguments, which are expected to provide the most informative evidence for the extraction of video events. In order to capture the visual state changes of arguments, we decompose them into changes in pixels within objects, displacements of objects, and interactions among multiple arguments. We further propose Object State Embedding, Object Motion-aware Embedding and Argument Interaction Embedding to encode and track these changes respectively. Experiments on various video event extraction tasks demonstrate significant improvements compared to state-of-the-art models. In particular, on verb classification, we achieve 3.49% absolute gains (19.53% relative gains) in F1@5 on Video Situation Recognition.

==> 0abstract.tex <==
\begin{abstract}

Video event extraction aims to detect salient events from a video and identify the arguments for each event as well as their semantic roles. 
Existing methods focus on capturing the overall visual scene of each frame, ignoring fine-grained argument-level information. 
Inspired by the definition of events as changes of  states, we propose a novel framework to detect video events by tracking the changes in the visual states of all involved arguments, which are expected to provide the most informative evidence for the extraction of video events. In order to capture the visual state changes of arguments, we decompose them into changes in pixels within objects, displacements of objects, and interactions among multiple arguments. We further propose Object State Embedding, Object Motion-aware Embedding and Argument Interaction Embedding to encode and track these changes respectively. Experiments on various video event extraction tasks demonstrate significant improvements compared to state-of-the-art models. In particular, on verb classification, we achieve 3.49\% absolute gains (19.53\% relative gains) in F\textsubscript{1}@5 on Video Situation Recognition.~\footnote[1]{Code and data resources are included in the supplementary materials and will be made publicly available for research purposes after publication. }
% by the changes in the state of all arguments and their interactions.
\end{abstract}

% In this paper, we argue that video events are discernible by the change in the visual state of all arguments, which actually provides the most convincing evidence for the extraction of video events.
%, and video events are indicatable by the changes in the state of all arguments and their interactions.
% we argue that visual state changes are the most indicative features to video event extraction, and video events are detectable by the changes in the state of all arguments and their interactions. %by state changes of all arguments. 
% Changes in visual state provide the most evidence for the extraction of video events
% Visual state changes are the most evidence for video event extraction, and all arguments and their interactions can be correlated with video events.
% we argue that visual state changes are the most indicative features of video event extraction, and video events can be predicted based on state changes in all arguments and the interactions between them.
% Visual changes are the most significant features when extracting video events, and video events can be predicted by the changes in the state of all arguments and their interactions.
% we argue that video events are indictable based on the sum of all arguments' state changes.
% we capture the argument visual state changes video events are indictable based on the sum of state changes of all arguments.

==> 1intro.tex <==
\section{Introduction}
% Situation Recognition~\cite{yatskar2016situation, pratt2020grounded} focuses on the ability of comprehending events, including the deep semantics of what is occurring, as well as the semantic roles of the involved objects.
The ability to comprehend a video requires a structured understanding of events, including what is happening, the objects involved, as well as their semantic roles. 
% As shown in Figure x, Video Situation Recognition~\cite{sadhu2021visual} aims to detect the \textit{knock} event where a man is run down by a bull. 
Situation Recognition~\cite{yatskar2016situation, pratt2020grounded} is a representative task for image event semantic structure understanding, aiming to classify an image to salient events (verbs)
%\heng{I don't think it's classified to one verb per image}\manling{Fixed. Situation Recognition only classifies the image/video to one verb, and call it as salient verb, but verb evaluation is based a ranking list. } 
and to predict entities (nouns) associated with semantic roles of each event. 
Video Situation Recognition~\cite{sadhu2021visual} extends the capacity of understanding event semantic structures from images to videos, as shown in Figure~\ref{img:task}. However, due to the high variation of temporal dynamics and visual features presented in videos, it remains to be a challenging and understudied task. 


\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.33]{AAAI 2023/image/example.png}
    \caption{An example of a video event, with \textsc{knock} as the verb and \textit{man} as \textsc{target(arg\textsubscript{1})}, \textit{bull} as \textsc{agent(arg\textsubscript{0})}. 
    \manling{add table structure}
    }
    \label{img:task}
\end{figure}

% The key challenge of video event understanding, compared to images, is the temporal tracking of objects and comparison of the state changes across frames. 
Traditional image event extraction~\cite{yatskar2016situation, pratt2020grounded,li2020cross,cho2022collaborative,wei2022rethinking} and video event extraction~\cite{medioni2001event,chen2021joint,sadhu2021visual} grasps the overall semantics of visual scenes, as a result of the difficulty in locating a specific visual area (i.e., a bounding box) to indicate the happening of an event. This is the case for images; however, additional temporal dynamics of videos provides another perspective to indicate the occurrences of events visually. 

% In terms of linguistic form and interpretation, events are referred to as telic and resultative.
% Events, in linguistic form and interpretation, are described to be telic and resultative, and are interpreted as state changes~\cite{dolling2008event}. 
Events, in linguistic form and interpretation, are telic, resultative, and indicate changes in states~\cite{dolling2008event}. 
% Linguistically, events are described as telic, resultative, and state-changing.
% We argue that video events naturally can be localized or indicatable by the changes in argument states, i.e., the sum of state changes of all arguments. 
Similarly, we argue that video events can, by nature, be represented by the visual state changes of all involved arguments. 
We further encode the \textbf{argument visual state changes} from three perspectives: (1) Single-frame state is characterized by in-bounding-box \textit{pixel changes} (such as the man's state changes from a running position to a lying position in Figure~\ref{img:task})  and \textit{displacements} of bounding boxes (such as the man moves from left to right in Figure~\ref{img:task}). 
% In-bounding-box state changes encode the \textit{pixel changes}, such as the man's state changes from a standing (running) position to a lying (defensive) position in Figure~\ref{img:task}; displacements capture the position changes, such as the bounding box of the man moves from left to right, and from big to small in Figure~\ref{img:task}. 
Therefore, we propose \textbf{Object State Embedding} (OSE) by encoding both pixel changes and displacements. %the \textit{pixel changes} inside the object bounding boxes (), as well as the \textit{displacement} of these objects;
% the \textit{displacements} of object bounding boxes, such as the bounding box of the man moves from left to right, and from big to small in Figure~\ref{img:task};  
(2) The motion of objects across multiple frames, which we introduce \textbf{Object Motion-aware Embedding} (OME) to 
aggregate the changes of object states from different frames. 
% \manling{the terminology is changed from 'object' to 'argument', a natural question will be how do you distinguish whether an object is an argument or not. Here we'd better add the gate for each object to decide whether include it or not, otherwise, we'd better just stick to one single terminology} 
(3) The interaction between objects, which we propose to learn an \textbf{Multi-Object Interaction Embedding} by encoding the interaction area,  which is able to capture the relative position of multiple objects and the pixel changes within intersection background. For example, the bounding boxes of \textit{man} and \textit{bull} are moving towards each other and then being apart, and the background pixels of \textit{grass} also indicate the  \textsc{knock down} event. %\textit{contextualizing} objects with other objects within the same scene, such as the man and the bull in Figure~\ref{img:task}. 
% \manling{I still think here should be the ``changes of interactions'', i.e., adding the tracking interaction changes (the union bounding boxes of all objects, including the environmental areas between objects) the same way as object state aggregator. We can see if we have time to add it later}. 

On top of that, the information of multiple objects and their interactions is aggregated by an \textbf{Argument Interaction Encoder}, by \textit{contextualizing} objects with other objects within the same scene, and learning to focus on the objects and interactions that are more indictable. For example, the \textit{man} and the \textit{bull} in Figure~\ref{img:task} are the major objects compared to the \textit{orange ring} in the background. 
%The event detection relies on the salient objects, which is learned to pay more attention to through the video event encoder.
With this module design, our proposed model learns to rely on the salient objects that are possibly important argument roles for event detection.

As a result of this new paradigm of video event formulation, %our verb classifier takes into account fine-grained states of arguments over time as well as their interactions.
we classify a salient verb for each video by taking into account fine-grained states of arguments over time, as well as their interactions. %based on capturing fine-grained argument states over time, as well as the interactions between them. 
% This new paradigm of video event formulation enables our verb classifier to take into account fine-grained states of arguments over time as well as their interactions.
% overall visual scene is decomposed into fine-grained argument states over time, as well as the interactions between them. 
The verb classification largely benefits from the joint modeling of multiple arguments, leading to 3.49\% absolute gains (19.53\% relative gains) in F\textsubscript{1}@5 according to the Video Situation Recognition validation set. Argument prediction enjoys a further boost due to the argument-level modeling, i.e., 3.97\% absolute gains on CIDEr.


Our contributions can be summarized as the follows:
\begin{itemize}
    % \setlength\itemsep{0em}
    \item We propose to formulate video events as the aggregation of visual state changes among multiple arguments. To the best of our knowledge, we are the first work to explore argument-level state changes in video event extraction. %or video situation recognition. 
    \item We propose a new encoding framework by decomposing state changes into in-bounding-box pixel changes, bounding-box displacements, and multi-argument interaction.  
    \item Experiment results on two tasks, verb classification and argument prediction, demonstrate significant improvements compared to state-of-the-art models.
\end{itemize}   

% Event extraction from unstructured plain text has become a popular and thoroughly-studied research topic,
% while due to the heterogeneity and inferiority of visual features,
% video event extraction remains to be a much more challenging task.
% In natural language processing domain,
% there are explicit event trigger words or verbs indicating the happening of events.
% However, when it comes to videos,
% only motions of objects implicitly convey the information of events. Meanwhile, arguments of an event are also represented as objects in a video. Inspired by this, we propose a novel model that tackles video event extraction by 
% encoding object state changes. 
% We design \textbf{Object State Embedding} (OSE) to 
% capture the object states and 
% design \textbf{Object Motion-aware Embedding} (OME) to
% characterize the motion of an object.
% \manling{change 'object' to 'argument'?}
% Furthermore, the OME of different objects are utilized by \textbf{Argument Interaction Encoder} to
% produce a visual event embedding, which is an overall description of the event in a video.
% We apply our model on VidSitu dataset~\cite{sadhu2021visual} which contains two event extraction tasks: verb classification and argument prediction, and achieve significant improvement.

% \manling{The previous version, language is really great:) but the logic is not quite clear. Using object state changes is not because that the motions of objects are equivalent to trigger words or verbs (which is hard to convince people), but because of the temporal dimension. }



==> 2model.tex <==
\section{Methodology}
Our goal is to identify events (verbs) in a video clip, and to fill in the semantic roles of each predicted verb with entities (nouns). Our main idea is to introduce argument-level information by encoding the state changes of all arguments via Object State Embeddings and Object Motion-aware Embeddings, as well as their interactions through Multi-object Interaction Embeddings (Section~\ref{sec:embedding}). 
Afterwards, all objects are globally contextualized via an Argument Interaction Encoder (Section~\ref{sec:encoder}) to pay attention to objects that might be of relevance to main arguments for verb classification (Section~\ref{sec:verb}) and semantic role prediction (Section~\ref{sec:argument}). 
%Then it is followed by an Argument Interaction Encoder to globally contextualize all objects with attention to objects that might be of relevance to main arguments (Section 3) for verb classification (Section 4) and semantic role prediction (Section 5). 
% In this section, we introduce our method in details. We first give the formal definition of the task, introduce each part of our model, and then demonstrate how to apply our model on two event extractions tasks: verb classification and semantic role prediction.



\subsection{Problem Formulation}

% Given a video clip $\mathcal{V}$ that last several seconds, the output is 
Given a video clip containing sampled frames $\{f_i\}_{i=0}^{F}$ with $F$ as the number of frames, the model is required to output a series of events $\{e\}$ occurring in the video. Each event is represented as a semantic structure
\begin{equation}
    e = \{v, 
    \langle r^0, a^0 \rangle, 
    \langle r^1, a^1 \rangle, 
    \cdots
    % , 
    % \langle r^m, a^m \rangle
    \},
\end{equation}
consisting a verb $v$ and multiple arguments $\{\langle r^k, a^k \rangle\}$ of the event. 
As defined in the event ontology, each verb $v$ is chosen from a pre-defined verb set $\mathcal{V}$, and has a pre-defined set of roles $\mathcal{R}(v)$. For example, the role set for the verb \textsc{knock} contains $\mathcal{R}(\textsc{knock})$ = $\{\textsc{agent}, \textsc{target}, \textsc{scene}, \dots\}$. $r^k \in \mathcal{R}(v)$ represents the $k$\textsuperscript{th} role of the verb $v$, and $a^k$ denotes the corresponding argument entity, which is described as a word or a phrase without a predefined set of words. 
% Each verb $v_i$ is chosen from a pre-defined verb set $\mathcal{V}$ in the event ontology.
% All verbs $v_i$ are chosen from a pre-defined verb set $\mathcal{V}$, while argument $A_i^j$ is a word or phrase describing the $j$-th role of the event $E_i$. 
% Take Figure~\ref{img:task} as an example. 
For example, the event detected for the video clip in Figure~\ref{img:task} is $v=$ \textsc{knock}, and main arguments are $\langle$\textsc{agent(arg\textsubscript{0})}, \textit{gray bull}$\rangle$, 
$\langle$\textsc{target(arg\textsubscript{1})}, \textit{midget in gray hoodie}$\rangle$ 
and 
$\langle$\textsc{place(arg\textsubscript{scene})}, \textit{ground}$\rangle$
, etc. \manling{update}



% \subsection{Object State Embedding \& Object Motion-aware Embedding}
% \subsection{Object State and Motion Change Tracking}
\subsection{Object Visual State Tracking}
\label{sec:embedding}
From the perspective of kinematics, the motion of an object can be decomposed into transitional and rotational movements, which correspond to the body shift and the rotation of the object, respectively.
Likewise, we apply this paradigm to videos and decompose the object motion into the \emph{displacement} of the bounding box and the \emph{pixel changes} within that bounding box.
% This paradigm can be applied to videos as well, allowing us to decompose motion into displacement of the bounding box and pixels changes within that bounding box.
As shown in Figure~\ref{fig:man_motion}, the displacement of the \textit{man} shows that he is moving from left to right and from near to far, while the pixel changes indicate that he is changing from standing to lying down. 
The motion of the \textit{man} can be well defined by the displacement of it bounding box and the pixel changes. Therefore, we detect objects in the video and propose object state embedding and object motion-aware embedding to encode the displacement and pixel changes of objects.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.4]{AAAI 2023/image/man_motion.png}
    \caption{Bounding boxes of a man in a video.}
    \label{fig:man_motion}
\end{figure}


\paragraph{Object Detection and Tracking} 
%To describe the displacement of an object's bounding box, we adopt VidVRD~\cite{gao2021video}, a state-of-the-art object tracking method, to generate object tracklets. 
We generate object tracklets using the state-of-the-art object tracking model VidVRD~\cite{gao2021video}. Taking a raw video as input, it outputs a list of object tracklets $\{o_j\}_{j=0}^{O}$, where $O$ is the number of recognized objects. 
Each object tracklet $o_j$ consists a list of its appearances in the video, and each apprearance is characterized by a time slot $\left[ t_{j}^{-}, t_{j}^{+} \right]$ and the coordinates of the left bottom and the right top corners of the bounding box 
\begin{equation}
    b_{ji} = \langle (b_{ji}^{0}, b_{ji}^{1}), (b_{ji}^{2}, b_{ji}^{3}) \rangle
\end{equation}
 at each time stamp inside the time slot. 
% Each $T_j$ with length (number of frame in which the object appears) $l_j$ is characterized by its time slot $(st_j, ed_j)$ and bounding box coordinates $\{b_{ji}\in \mathbb{R}^4|i=st_j,\dots, ed_j\}$.
Take Figure~\ref{fig:man_motion} as an example. The object \textit{man} is detected on four frames with the bounding boxes extracted from each frame. 
% In four sample video frames, 

\paragraph{Video Encoding Backbone} 
To utilize the superior power of 3D convolutional neural networks and improve computation efficiency,
our object state and motion-aware embedding use the state-of-the-art SlowFast model \cite{feichtenhofer2019slowfast} as the video encoder to get high-level grid features of raw videos. 
It includes a Slow pathway operating at a low frame rate to encode spatial semantics, and a Fast pathway operating at a high frame rate to capture motion at fine temporal resolution. %is used as a video encoder to get high-level grid features of raw videos.

The video encoder takes as input slow and fast sampled video frames $f^{\text{slow}}\in \mathbb{R}^{F_1\times W \times H \times 3}$ and $ f^{\text{fast}}\in \mathbb{R}^{F_2 \times W \times H \times 3}$, 
and outputs slow and fast grid features $\bs{g}^{\text{slow}}\in \mathbb{R}^{F_1\times W' \times H' \times d_1},
\bs{g}^{\text{fast}} \in \mathbb{R}^{F_2 \times W' \times H' \times d_2}$:
\begin{equation}
    [\bs{g}^{\text{slow}}, \bs{g}^{\text{fast}}] = \mathrm{SlowFast}(f^{\text{slow}}, f^{\text{fast}}),
\end{equation}
where 
$F_1$ and $F_2$ are the number of frames sampled from the video in slow and fast pathways, with the constraint of $F_1 < F_2$. Here, $W$ and $H$ are the width and height of raw video frames,
with $W'$ and $H'$ as the width and height of the processed grid features.
% Notice that $F_1 < F_2$ and both of them are the number of frames sampled from the video,
$d_1$ and $d_2$ are the number of channels of slow and fast grid features respectively.


\paragraph{Single Frame: Object State Embedding} 
First, in order to encode the states of objects in each frame, we introduce Object State Embedding. As shown in Figure~\ref{fig:man_motion}, we decompose the object state into in-bounding-box pixels for visual state tracking, as well as the position of the bounding box for displacement tracking. 

Given an object $o_j$ in a video frame $f_i$ and its appearance bounding box $b_{ji} = \langle (b_{ji}^{1}, b_{ji}^{2}), (b_{ji}^{3}, b_{ji}^{4}) \rangle$, we first project the corresponding bounding box to the grid feature space $ \hat b_{ji} = \langle (\hat b_{ji}^{1}, \hat b_{ji}^{2}), (\hat b_{ji}^{3}, \hat b_{ji}^{4}) \rangle$ by normalizing the coordinates.
To encode the state of the object $o_j$, we mask grid features outside the bounding box and exclusively focus on the object.
% exclusively focus on the in-bounding-box pixels and the position of the object. 
% Now, we focus on the grid feature $\bs{g}$.
% Given the bounding box of an object in a frame of the raw video, we first calculate the corresponding bounding box in the grid feature space, then we mask all grid features outside the bounding box
% and only focus on the location and in-bounding-box grid features.

% Following the displacement plus pixel changes paradigm,
% the state of the object can be characterized as the coordinates of bounding box 
% and the grid features within the bounding box.
% Therefore,
% as shown in figure \ref{fig:state}, we define the \textbf{object state embedding} as 
% the concatenation of in-bounding-box grid feature average and coordinates positional embedding,
% which represents the state of the object.
% % The remaining part is exactly in-bounding-box pixels with their location,
% % which means the masked video represents \emph{displacement} and \emph{pixel changes} of the object.

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{AAAI 2023/image/state_embeding.pdf}
    \caption{State embedding of the man in the first frame.}
    \label{fig:state}
\end{figure}

The visual state of an object $o_j$ is determined by its current status presented in the  frame $f_i$, such as the running status in Figure~\ref{fig:man_motion}. Thus, we adopt average pooling over the grid features within the bounding box: 
% \xudong{I feel pixel-wise could be confusing as they may think this is averaged raw pixels. How about simply call it pooled feature? We need to change every pixel average accordingly if we decide another name, include Figure 3. or maybe we cn clarify in figure 3 that pixels here are actually representated as feature vectors}
%$\langle (\hat b_{ji}^{1}, \hat b_{ji}^{2}), (\hat b_{ji}^{3}, \hat b_{ji}^{4}) \rangle$ 
% as the representative features for the current visual state
% Formally, the in-bounding-box pixel feature $\bs{p}_{ji}$ is defined as:
\begin{equation}
    \begin{aligned}
\bs{p}_{ji} & = \frac 1{(\hat b^{2}_{ji}-\hat b^{0}_{ji})(\hat b^{3}_{ji}-\hat b^{1}_{ji})} \sum_{x =\hat b^{0}_{ji}}^{\hat b^{2}_{ji}-1} \sum_{y = \hat b^{1}_{ji}}^{\hat b^{3}_{ji}-1} \bs{g}_{i}[x,y]. 
\end{aligned}
\end{equation}
where $(\hat b^{0}_{ji}, \hat b^{1}_{ji})$ and $(\hat b^{2}_{ji}, \hat b^{3}_{ji})$ represent the left bottom and the right top corners of the bounding box. $\bs{g}_{i}[x,y]$ represents the grid feature of the coordinate $\langle x,y \rangle$ in the grid feature space. The grid features $\bs{g}_{i}$ are from the slow pathway ($\bs{p}_{ji}^{\text{slow}} \in \mathbb{R}^{d_{1}}$) and the fast pathway ($\bs{p}_{ji}^{\text{fast}} \in \mathbb{R}^{d_{2}}$).  
%$\bs{p}_{ji}^{\text{slow}} \in \mathbb{R}^{d_{1}}$ is based on the grid features $\bs{g}_{i}^{\text{slow}}$ o.


To track the displacement of the object $o_j$, we encode its coordinates to track position changes: 
\begin{equation}
    \begin{aligned}
\bs{c}_{ji} & = \bs{W}_c\hat b_{ji},
\end{aligned}
\end{equation}
where $\bs{c}_{ji} \in \mathbb{R}^{d_c}$ is the coordinate embedding, with $d_c$ as its dimension. $\bs{W}_{c} \in \mathbb{R}^{d_{c} \times 4}$ is a positional embedding. 

% Formally speaking, we denote $f_i \in \mathbb{R}^{W'\times H' \times F}$ as the slow or fast
% grid feature of frame $i$.
% Also, we assume left bottom and right top corners of the bounding box of object $j$ in grid feature space are $(\hat b^{0}_{ji}, \hat b^{1}_{ji})$ and $(\hat b^{2}_{ji}, \hat b^{3}_{ji})$.

As a result, the \textit{Object State Embedding} (OSE) $\bs{s}_{ji} \in \mathbb{R}^{d+d_c}$ is defined as the concatenation of pooled features $\bs{p}_{ji}$ and coordinate-based features $\bs{c}_{ji}$:
\[
\begin{aligned}
% c_{ji} & = W_c\hat b_{ji} \\
% p_{ji} & = \frac 1{(\hat b^{2}_{ji}-\hat b^{0}_{ji})(\hat b^{3}_{ji}-\hat b^{1}_{ji})} \sum_{x =\hat b^{0}_{ji}}^{\hat b^{2}_{ji}-1} \sum_{y = \hat b^{1}_{ji}}^{\hat b^{0}_{ji}-1} f_{i,x,y} \\
\bs{s}_{ji} & = [\bs{p}_{ji}, \bs{c}_{ji}]. 
\end{aligned}
\]

% \noindent where $c_{ji} \in \mathbb{R}^{d_c}$ is the coordinate embedding, with $d_c$ as its dimension. 
% $p_{ji}\in \mathbb{R}^{F}$ and $ose_{ji} \in \mathbb{R}^{F+C}$ are the coordinate, pixel average and object state embedding.
% $W_{c} \in \mathbb{R}^{C \times 4}$ is a positional embedding layer and $C$ is a hyper-parameter.



\paragraph{Multiple Frames: Object Motion-aware Embedding} 
To track the state changes of an object $o_j$ across multiple frames $\{f_i\}_{i=0}^{F}$ along the temporal dimension,
we feed object state embeddings of these frames into an \emph{object state aggregator}
%which could be any sequential model capable of capturing the differences among state embeddings.
to capture their differences, as shown in Figure~\ref{fig:motion_embedding}. 
% Therefore, the output of the model would be an embedding containing all information about the object's motion, which we define as \textbf{object motion-aware embedding}. This process is shown below in figure \ref{fig:motion_embedding}.
% This object motion-aware embedding enables the model 
It enables the model to capture the motion of the object $o_j$ when the video unfolds, so we call it \textit{Object Motion-aware Embedding} (OME) $\bs{m}_j$:  
% To elaborate, the object motion-aware embedding is defined as 
\begin{equation}
    \bs{m}_j = \mathrm{StateAgg}(\{\bs{s}_{ji}\}_{i=0}^{F} ),
\end{equation}
where 
%$ose_j\in \mathbb{R}^{T\times(d+d_c)}$ is the object state embedding, and 
$\bs{m}_j \in \mathbb{R}^{d+d_c}$. 
The encoding is also done for both slow and fast pathways, i.e., $\bs{m}_j^{\text{slow}} \in \mathbb{R}^{d_1+d_c}, \bs{m}_j^{\text{fast}}\in \mathbb{R}^{d_2+d_c}$ respectively. 

Regarding the object state aggregator, we adopt LSTM~\cite{hochreiter1997long} as well as average pooling, and  perform further ablation studies on the choice of the aggregation operator. %. The results support that average pooling is powerful enough.
% We adopt 

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{AAAI 2023/image/aggregator.pdf}
    \caption{Object Motion-aware Embedding and Object Interaction Embedding.}
    \label{fig:motion_embedding}
\end{figure}

% Since the encoder gives slow and fast grid feature, we will get both slow and fast object motion-aware embedding $ome_j^{\text{slow}} \in \mathbb{R}^{F_1+C}, ome_j^{\text{fast}}\in \mathbb{R}^{F_2+C}$ respectively.



\paragraph{Multiple Objects: Object Interaction Embedding}

Apart from the motion of individual objects,
we further explore the joint state changes of multiple objects. % great factor we need to consider is the interaction between objects.
As one example, the interaction between the \textit{man} and the \textit{bull} in Figure~\ref{fig:motion_embedding} contains the changes of relative positions by moving towards each other, then overlapping, and finally moving far apart. Also, the pixel changes of the interaction area between the \textit{man} and the \textit{bull}  provide a context, such as the building, the ground, the falling down circle ring, etc. 
% That is, OME only focuses on the \emph{intra-bounding-box} changes
% while the object interactions are the \emph{inter-bounding-box} changes.
% To illustrate, in the ``bull-knock-man'' event, only when the model knows that the target of the bull is the man will it give the correct extraction of the event.
We therefore propose {Object Interaction Embedding} to capture and track changes to the interaction area across objects.
% Therefore, we propose \textbf{Object Interaction Embedding} (OIE) to capture the interaction area across objects, as well as tracking its changes.

To reveal an overall picture of how objects interact in a video frame $f_i$,
we first get the union bounding box $\hat{B}_i$ of these objects: 
\begin{equation}
    \hat{B}_i = \bigcup_{o_j \in \mathcal{O}_i} \hat{b}_{ji}
\end{equation}
where $\mathcal{O}_i$ is the set of objects in frame $f_i$ and $\cup$ computes the union of their bounding boxes.
Since the interaction area can also be characterized by the pixel changes and position changes, we use similar approach as OME to construct interaction states by the grid features within the interaction area: 
\begin{equation}
    \bs{p}'_{i} = \frac 1{(\hat B^{2}_{i}-\hat B^{0}_{i})(\hat B^{3}_{i}-\hat B^{1}_{i})} \sum_{x =\hat B^{0}_{i}}^{\hat B^{2}_{i}-1} \sum_{y = \hat B^{1}_{i}}^{\hat B^{3}_{i}-1} \bs{g}_{i}[x,y],
\end{equation}
and the coordinates showing the position of the area:  
\begin{equation}
\bs{c}'_{i} = \bs{W}_c\hat B_{i}.
\end{equation}
Similarly we represent the state of the interaction area of frame $f_i$ via a concatenation operation to gather information of both perspectives:
\begin{equation}
    \bs{i}_{i} = [\bs{p}'_{i}, \bs{c}'_{i}],
\end{equation}
where $\bs{i}_i \in \mathbb{R}^{d+d_c}$
After that, we employ an interaction aggregator to track the state changes of the interaction area as \textit{Object Interaction Embedding} (OIE) $\bs{i} \in \mathbb{R}^{d+d_c}$: 
\begin{equation}
    \bs{i} = \mathrm{InterAgg}(\{\bs{i}_{i}\}_{i=0}^{F}), 
\end{equation}
where $\mathrm{InterAgg}$ follows the same architecture as $\mathrm{StateAgg}$.
% \noindent where $e_{\text{inter.}}$ is the Object Interaction Embedding and 
% for convenience, $\mathrm{InterAgg}$ uses the same architecture as $\mathrm{StateAgg}$.
% \manling{are StateAgg and InterAgg are the same parameters?}
Notice that we get $\bs{i}^{\text{slow}} \in \mathbb{R}^{d_1+d_c}$ 
and $\bs{i}^{\text{fast}} \in \mathbb{R}^{d_2+d_c}$ through the slow and fast pathways, respectively. 
% Similarly, we concatenate both pathways and shrink the dimension to $\bs{i} \in \mathbb{R}^{\frac{1}{\alpha}(d_1+d_2)}$.


\subsection{Argument Interaction Encoder}
\label{sec:encoder}


Considering that not all state changes objects are relevant to the occurrence of the event, we contextualize each object in the video, 
% \heng{I don't understand what this means: "globally contextualize the objects over other objects"} 
and ask the model to learn to pay attention to the objects that are most relevant to the video and other objects. 
% In a gesture to incorporate knowledge from OME into our model and gather all of the motion information of arguments, we design the argument interaction encoder to capture the interactions between different arguments or objects.
Therefore, we employ a Transformer layer \cite{vaswani2017attention} taking as input the overall embedding of entire video, the Object Motion-aware Embedding (OSE) $\{\bs{m}_{j}\}_{j=0}^{O}$ of candidate objects,
and the Object Interaction Embedding (OIE) $\bs{i}$ of the interaction area: 
\begin{equation}
    \bs{e} = \mathrm{Trans}(\ [\overline{\bs{g}}; \  \{\bs{m}_{j}\}_{j=0}^{O}; \  \bs{i}]\ ),
\end{equation}
where $\overline{\bs{g}} \in \mathbb{R}^{d}$ is the average-pooled features over all frames, and is used to represent the overall semantics of the video. 
The maximum number of objects $O$ is set as a hyperparameter, and the objects are ranked in terms of the confidence from the object detector.
It enables the output embedding to encode representative information to determine the event semantic structures, so we call it  \textit{event-aware visual embedding} $\bs{e}$.
% ,  and can be used to support a variety of tasks that requires event understanding, such as  
% which contains all the visual information about the event.
% For example, in the ``bull-knock-man'' video, we have
% \[
% \begin{aligned}
% e_{\text{all}}^p & = \frac 1{WH} \sum_{x = 0}^{W} \sum_{y = 0}^H f_{p, i, x, y},\quad  p\in\{\text{slow, fast}\} \\
% e_{q} & = [e_q^\text{ slow}, e_q^\text{fast}], \quad q \in \{\text{all, inter}\} \\
% ome_j & = [ome_j^\text{slow}, ome_j^\text{fast}], \quad j \in \{\text{bull}, \text{man}\}\\
% \\
% \end{aligned},
% \]
For each embedding $\overline{\bs{g}}$, $\bs{m}_{j}$ and $\bs{i}$, we concatenate their embeddings from both slow and fast pathways, and further project $\bs{e} \in \mathbb{R}^{3d_1+3d_2+2d_c}$ to $\bs{e} \in \mathbb{R}^{d_1+d_2}$ using a linear layer. 
% To , and we further shrink their dimensions to $\bs{m}_j \in \mathbb{R}^{\frac{1}{\alpha}(d_1+d_2)}$ with a linear layer, for better alignment in argument interaction encoder. Here $\alpha$ is a hyper-parameter and we set it to 3.
% Here, $\overline{\bs{g}} \in \mathbb{R}^{d_1+d_2}$ is splitted into $\alpha$ tokens
% and $\bs{e} \in \mathbb{R}^{d_1+d_2}$ is the concatenation of first $\alpha$ tokens of the output.

% The final model is shown in Figure \ref{fig:model}. The event-aware visual embedding is designed for various tasks including verb classification, argument prediction and co-referencing.

\begin{figure}
    \centering
    \includegraphics[scale=0.53]{AAAI 2023/image/overview.pdf}
    \caption{An overview of our event-aware visual embedding.}
    \label{fig:model}
\end{figure}



\subsection{Verb Classification}
\label{sec:verb}
Verb classification is a rudiment motion-related video understanding task to select verbs $\{v\}$ from a predefined event ontology\footnote{There are 2154 verb-senses defined in the event ontology of the video situation recognition dataset  VidSitu~\cite{sadhu2021visual}.}. Our event-aware visual embedding $\bs{e}$ captures the state changes of arguments, which is the most informative feature to identify events. 
As a result, we classify the video by 
% where given a video clip, our model is required to classify the verb for the most salient event in the clip.
% We follow the standard in VidSitu: non-visual and fine-grained verb-senses are manually discarded  and there are in total 	2154 verb-senses for classification.
% As our event-aware visual embedding provides a more overall understanding about an event and what's happening in the video, we believe our model could achieve higher performance.
% The model architecture is simple:
feeding its event-aware visual embedding $\bs{e}$ into a classification layer
and train our model with a cross-entropy loss following~\cite{sadhu2021visual}.
The classification layer consists of two linear transformations 
with a ReLU activation layer in between:
\begin{equation}
    v = \mathrm{Softmax} \left( \bs{W}_2 \ \left[ \mathrm{ReLU} \ ( \bs{W}_1 \bs{e} + \bs{b}_1) \right] + \bs{b}_2 \right),
\end{equation}
which produces a ranked list of the predicted verb $v$ based on the $\mathrm{Softmax}$ probabilities. We set the bottleneck dimension to $\frac{1}{2} (d_1+d_2)$, namely,
$\bs{W}_1:\mathbb{R}^{d_1+d_2} \to \mathbb{R}^{\frac{1}{2} (d_1+d_2)}$
and $W_2: \mathbb{R}^{\frac{1}{2} (d_1+d_2)} \to \mathbb{R}^{|\mathcal{V}|}$,
where $\mathcal{V}$ is the set of candidate verbs defined in the event ontology.



\subsection{Semantic Role Prediction}
\label{sec:argument}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.43]{AAAI 2023/image/decoder.pdf}
    \caption{An overview of our model for semantic role prediction. 
    % \manling{remove the global contextulization, not important but a distraction. can be in appendix}
    }
    \label{fig:arg_model}
\end{figure}

The most challenging part of event semantic structure extraction is to recognize the involved objects and their semantic roles. 
% The state-of-the-art model~\cite{sadhu2021visual} utilizes a sequence-to-sequence framework to decode the arguments 
Our event-aware visual embedding $\bs{e}$ preserves fine-grained argument-level information, so we follow the architecture of state-of-the-art  model~\cite{sadhu2021visual} but replace its input SlowFast embedding with our event-aware visual embedding $\bs{e}$.      
% In order to test the fidelity of argument information contained in the event-aware visual embedding, given verbs for every 2-second clip,  our model is required to predict the arguments of the event.
% We still follow the baseline seq-to-seq model from \cite{sadhu2021visual}, except that $e_{\text{event}}$ are used as the input for transformer encoder.
In detail, the arguments are decoded in a sequence-to-sequence manner shown in Figure~\ref{fig:arg_model}, where the decoded sequence is the concatenation of the verb and its arguments 
% ``\textsc{verb} \texttt{[Arg$_{0}$]} \textsc{noun} \texttt{[Arg$_{1}$]} \textsc{noun} ...''.
``$v$ \texttt{[Arg$_{0}$]} $a^{0}$ \texttt{[Arg$_{1}$]} $a^{1}$ ...'', namely, the $k$\textsuperscript{th} argument $a^{k}$ is predicted by: 
\begin{equation}
    a^{k} = \mathrm{Decoder}(v \left[\text{\texttt{Arg}}_{0}\right] a^0 \left[\text{\texttt{Arg}}_{1}\right] a^1 \cdots \left[\text{\texttt{Arg}}_{k}\right]). %$a^{0}$ \texttt{[Arg$_{1}$]} $a^{1}$ ...'')
\end{equation}
Our training objective is cross entropy loss between the generated sequence and the ground-truth sequence. We use teacher forcing strategy to obtain the verb $v$ during training. 
% We freeze (?)

% Because the object and argument information are encoded into the event-aware visual embedding, we believe that it is easier to decode the correct argument for the model.

%\subsection{Event Contrastive Loss}

%When it comes to injecting the textual event knowledge into a visual model,
%we propose the event contrastive loss to align visual and textual event information.
%To elaborate,
%on the visual side,
%we've obtained the OME for every object in the video,
%while with the help of modern pre-trained language model,
%we can extract an event-entity graph from the textual labels.
%Based on the assumption that the visual event is the sum of all its arguments' states changing,
%the event contrastive loss is designed 
%to align the sum of all visual objects' OME 
%and the sum of all textual arguments' embedding,
%as shown in figure \ref{fig:event_contrastive}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.25]{AAAI 2023/image/event_contrastive.png}
%    \caption{Computation of event contrastive loss.}
%    \label{fig:event_contrastive}
%\end{figure}

%The negative example for event contrastive loss
%would be other textual events from the same training batch,
%which means if the visual and textual embedding describe the same event,
%we make them close to each other.


==> 2model_bak.tex <==
\section{Methodology}
Our goal is to identify events (verbs) in a video clip, and to fill in the semantic roles of each predicted verb with entities (nouns). Our primary idea is to introduce argument-level information by encoding the state changes of all arguments via Object State Embeddings and Object Motion-aware Embeddings, as well as their interactions through Multi-object Interaction Embeddings (Section~\ref{sec:embedding}). 
Afterwards, all objects are globally contextualized via an Argument Interaction Encoder (Section~\ref{sec:encoder}) to pay attention to objects that might be of relevance to main arguments for verb classification (Section~\ref{sec:verb}) and semantic role prediction (Section~\ref{sec:argument}). 
%Then it is followed by an Argument Interaction Encoder to globally contextualize all objects with attention to objects that might be of relevance to main arguments (Section 3) for verb classification (Section 4) and semantic role prediction (Section 5). 
% In this section, we introduce our method in details. We first give the formal definition of the task, introduce each part of our model, and then demonstrate how to apply our model on two event extractions tasks: verb classification and semantic role prediction.

\begin{comment}
Event extraction from unstructured plain text has become a popular and thoroughly-studied research topic,
while due to the heterogeneity and inferiority of visual features,
video event extraction remains to be a much more challenging task.
In natural language processing domain,
there are explicit event trigger words or verbs indicating the happening of events.
However, when it comes to visual event,
only implicit and subtle motion of objects are related to it.
Considering this status quo,
our model is designed to tackle video event extraction by 
encoding argument state changes,
which perfectly matches the definition of events.

Arguments of an event are represented as objects in a video,
so we model the argument state changes as object state changes,
or object motion.
Consequently, sum of all object motion 
naturally contains all information about the event.

Inspired by this intuition, we propose \textbf{Object State Embedding} to 
capture the object states and 
design \textbf{Object Motion-aware Embedding} (OME) to
characterize the motion of an object.
Furthermore, the OME of different objects are utilized by \textbf{Argument Interaction Encoder} to
produce a visual event embedding, which is an overall description of the event in a video.
\end{comment}

\subsection{Problem Formulation}

% Given a video clip $\mathcal{V}$ that last several seconds, the output is 
Given a video clip $V$, the model is required to output a series of events $\{E_1, E_2, \cdots, E_k\}$ occurring in the video. Each event is represented as a semantic structure 
\begin{equation*}
    E_i = \{v_i, 
    \langle r_i^1, a_i^1 \rangle, 
    \langle r_i^2, a_i^2 \rangle, 
    \cdots, 
    \langle r_i^m, a_i^m \rangle
    \},
\end{equation*}
consisting a verb $v_i$ and multiple arguments $\{\langle r_i^j, a_i^j \rangle\}$ of the event. As defined in the event ontology, each verb $v_i$ is chosen from a pre-defined verb set\footnote{There are 1500 unique verbs defined in the event ontology of the video situation recognition dataset  VidSitu~\cite{sadhu2021visual}.} $\mathcal{V}$, and has a pre-defined set of roles $\mathcal{R}(v_i)$. Here, $r_i^j \in \mathcal{R}(v_i)$ represents the $j$\textsuperscript{th} role of the verb $v_i$, and $a_i^j$ denotes the corresponding argument entity, which an open-word word or phrase. 
% Each verb $v_i$ is chosen from a pre-defined verb set $\mathcal{V}$ in the event ontology.
% All verbs $v_i$ are chosen from a pre-defined verb set $\mathcal{V}$, while argument $A_i^j$ is a word or phrase describing the $j$-th role of the event $E_i$. 
% Take Figure~\ref{img:task} as an example. 
For example, the event detected for the video clip in Figure~\ref{img:task} is \textsc{knock}, and main arguments are $\langle$\textsc{agent}, \textit{gray bull}$\rangle$, 
$\langle$\textsc{target}, \textit{midget in gray hoodie}$\rangle$ 
and 
$\langle$\textsc{scene}, \textit{ground}$\rangle$.



% \subsection{Object State Embedding \& Object Motion-aware Embedding}
% \subsection{Object State and Motion Change Tracking}
\subsection{Object Visual State Tracking}
\label{sec:embedding}
From the perspective of kinematics, the motion of an object can be decomposed into transitional and rotational movements, which correspond to the body shift and the rotation of the object, respectively.
Likewise, we apply this paradigm to videos and decompose the object motion into the \emph{displacement} of the bounding box and the \emph{pixel changes} within that bounding box.
% This paradigm can be applied to videos as well, allowing us to decompose motion into displacement of the bounding box and pixels changes within that bounding box.
As shown in Figure~\ref{fig:man_motion}, the displacement of the \textit{man} shows that he is moving from left to right and from near to far, while the pixel changes indicate that he is changing from standing to lying down. 
The motion of the \textit{man} can be well defined by the displacement of it bounding box and the pixel changes. Therefore, we detect objects in the video and propose object state embedding and object motion-aware embedding to encode the displacement and pixel changes of objects.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.4]{AAAI 2023/image/man_motion.png}
    \caption{Bounding boxes of a man in a video.}
    \label{fig:man_motion}
\end{figure}


\paragraph{Object Detection and Tracking} 
%To describe the displacement of an object's bounding box, we adopt VidVRD~\cite{gao2021video}, a state-of-the-art object tracking method, to generate object tracklets. 
We generate object tracklets using the state-of-the-art object tracking model VidVRD~\cite{gao2021video}. Taking a raw video as input, it outputs a list of object tracklets $\{T_j\}_{j=1}^n$, where $n$ is the number of recognized objects. Each $T_j$ with length (number of frame in which the object appears) $l_j$ is characterized by its time slot $(st_j, ed_j)$ and bounding box coordinates $\{b_{ji}\in \mathbb{R}^4|i=st_j,\dots, ed_j\}$.

\paragraph{Video Encoding Backbone} 
To utilize the superior power of 3D convolutional neural networks and improve computation efficiency,
our object state and motion-aware embedding are built upon the state-of-the-art SlowFast model \cite{feichtenhofer2019slowfast},
which is used as a video encoder to get high-level grid features of raw videos.

The video encoder takes as input slow and fast sampled video frames $v_{\text{slow}}\in \mathbb{R}^{T_1\times W \times H \times 3}, v_{\text{fast}}\in \mathbb{R}^{T_2 \times W \times H \times 3}$
and outputs slow and fast grid features $f_{\text{slow}}\in \mathbb{R}^{T_1\times W' \times H' \times F_1},
f_{\text{fast}} \in \mathbb{R}^{T_2 \times W' \times H' \times F_2}$:
\[
    [f_{\text{slow}}, f_{\text{fast}}] = \mathrm{SlowFast}(v_{\text{slow}}, v_{\text{fast}}),
\]
where $W$ and $H$ are the width and height of raw video frames,
and $W'$ and $H'$ are the width and height of the processed grid features.
Notice that $T_1 < T_2$ and both of them are the number of frames sampled from the video,
while $F_1, F_2$ are the number of channels of slow and fast grid features respectively.


\paragraph{Object State Embedding} Now, we focus on the grid feature $f$.
Given the bounding box of an object in a frame of the raw video, we first calculate the corresponding bounding box in the grid feature space, then we mask all grid features outside the bounding box
and only focus on the location and in-bounding-box grid features.
Following the displacement plus pixel changes paradigm,
the state of the object can be characterized as the coordinates of bounding box 
and the grid features within the bounding box.
Therefore,
as shown in figure \ref{fig:state}, we define the \textbf{object state embedding} as 
the concatenation of in-bounding-box grid feature average and coordinates positional embedding,
which represents the state of the object.
% The remaining part is exactly in-bounding-box pixels with their location,
% which means the masked video represents \emph{displacement} and \emph{pixel changes} of the object.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{AAAI 2023/image/object_state.png}
    \caption{State embedding of the man in the first frame.}
    \label{fig:state}
\end{figure}

Formally speaking, we denote $f_i \in \mathbb{R}^{W'\times H' \times F}$ as the slow or fast
grid feature of frame $i$.
Also, we assume left bottom and right top corners of the bounding box of object $j$ in grid feature space are $(\hat b^{0}_{ji}, \hat b^{1}_{ji})$ and $(\hat b^{2}_{ji}, \hat b^{3}_{ji})$.
Then, the object state embedding would be:

\[
\begin{aligned}
c_{ji} & = W_c\hat b_{ji} \\
p_{ji} & = \frac 1{(\hat b^{2}_{ji}-\hat b^{0}_{ji})(\hat b^{3}_{ji}-\hat b^{1}_{ji})} \sum_{x =\hat b^{0}_{ji}}^{\hat b^{2}_{ji}-1} \sum_{y = \hat b^{1}_{ji}}^{\hat b^{0}_{ji}-1} f_{i,x,y} \\
ose_{ji} & = [p_{ji}, c_{ji}] \\
\end{aligned},
\]

\noindent where $c_{ji} \in \mathbb{R}^{C}$, $p_{ji}\in \mathbb{R}^{F}$ and $ose_{ji} \in \mathbb{R}^{F+C}$ are the coordinate, pixel average and object state embedding.
$W_{c} \in \mathbb{R}^{C \times 4}$ is a positional embedding layer and $C$ is a hyper-parameter.
We keep $C = 128$ in our experiments.


\paragraph{Object Motion-aware Embedding} To track the state changes of an object,
we feed the state embeddings of the object into an \emph{object states aggregator},
which could be any sequential model capable of capturing the differences among state embeddings.
Therefore, the output of the model would be an embedding containing all information about 
the object's motion, which we define as \textbf{object motion-aware embedding}.
This process is shown below in figure \ref{fig:motion_embedding}.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.26]{AAAI 2023/image/motion_embedding.png}
    \caption{Object motion-aware embeddings of the man and bull in the video.}
    \label{fig:motion_embedding}
\end{figure}

To elaborate,
the object motion-aware embedding is defined 
as $ome_j = \mathrm{StateAgg}(ose_j)$, where $ose_j\in \mathbb{R}^{T\times(F+C)}$ is the object state embedding,
and $ome_j \in \mathbb{R}^{F+C}$ is the object motion-aware embedding.
Regarding the object state aggregator,
we tried LSTM \cite{hochreiter1997long} and simple average pooling.
The results support that average pooling is powerful enough.

Since the encoder gives slow and fast grid feature, 
we will get both slow and fast object motion-aware embedding 
$ome_j^{\text{slow}} \in \mathbb{R}^{F_1+C}, ome_j^{\text{fast}}\in \mathbb{R}^{F_2+C}$ respectively.

The overall dimension of OME is shrunk to $\frac{F_1+F_2}{\alpha}$ with a linear layer,
for better alignment in argument interaction encoder.
Here $\alpha$ is a hyper-parameter and we set it to 3.

\paragraph{Object Interaction Embedding}
Except for objects' individual motion,
another great factor we need to consider is the interaction between objects.
That is, OME only focuses on the \emph{intra-bounding-box} changes
while the object interactions are the \emph{inter-bounding-box} changes.
To illustrate,
in the ``bull-knock-man'' event,
only when the model knows that the target of the bull is the man will it give the correct extraction of the event.
Therefore, we propose \textbf{Object Interaction Embedding} (OIE) to capture the interaction changes.

To reveal an overall picture of containing all objects,
we first get the union of all bounding box: $\hat{B}_i = \bigcup_{j \in O_i} \hat{b}_{ji}$,
where $O_i$ is the objects' indices in frame $i$ and $\cup$ computes the union of all bounding boxes.
Following the approach to get OME, 
we also construct interaction states and use an interaction aggregator to calculate the OIE:

\[
\begin{aligned}
c_{i} & = W_c\hat B_{i} \\
p_{i} & = \frac 1{(\hat B^{2}_{i}-\hat B^{0}_{i})(\hat B^{3}_{i}-\hat B^{1}_{i})} \sum_{x =\hat B^{0}_{i}}^{\hat B^{2}_{i}-1} \sum_{y = \hat B^{1}_{i}}^{\hat B^{0}_{i}-1} f_{i,x,y} \\
ie_{i} & = [p_{i}, c_{i}] \\
e_{\text{inter.}} & = \mathrm{InterAgg}(ie) \\
\end{aligned},
\]

\noindent where $e_{\text{inter.}}$ is the Object Interaction Embedding and 
for convenience, $\mathrm{InterAgg}$ uses the same architecture as $\mathrm{StateAgg}$.
Notice that we can also get $e_{\text{inter.}}^{\text{slow}}$ 
and $e_{\text{inter.}}^{\text{fast}}$.
Concatenate them and shrink the dimension, and we'll get $e_{\text{inter.}} \in \mathbb{R}^{\frac{F_1+F_2}{\alpha}}$.


\subsection{Argument Interaction Encoder}
\label{sec:encoder}
In a gesture to incorporate knowledge from OME into our model
and gather all of the motion information of arguments,
we design the argument interaction encoder to capture the interactions between different arguments or objects.
The encoder is a single-layer Transformer \cite{vaswani2017attention} taking as input the whole video, the OME of all objects,
and the interaction embedding.
The output of the encoder is a visual event embedding $e_\text{event}$
which contains all the visual information about the event.
For example, in the ``bull-knock-man'' video, we have
\[
\begin{aligned}
e_{\text{all}}^p & = \frac 1{WH} \sum_{x = 0}^{W} \sum_{y = 0}^H f_{p, i, x, y},\quad  p\in\{\text{slow, fast}\} \\
e_{q} & = [e_q^\text{ slow}, e_q^\text{fast}], \quad q \in \{\text{all, inter}\} \\
ome_j & = [ome_j^\text{slow}, ome_j^\text{fast}], \quad j \in \{\text{bull}, \text{man}\}\\
e_{\text{event}} & = \mathrm{TransformerLayer}([e_{\text{all}}; ome_{\text{man}}; ome_{\text{bull}}; e_{\text{inter.}}]) \\
\end{aligned},
\]
where $e_{\text{all}}\in \mathbb{R}^{F_1+F_2}$ is splitted into $\alpha$ tokens
and $e_{\text{event}} \in \mathbb{R}^{F_1+F_2}$ is the concatenation of first $\alpha$ tokens of the output.

The final model is shown in figure \ref{fig:model}.
The visual event embedding is designed for various tasks
including verb classification, argument prediction and co-referencing.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{AAAI 2023/image/final_model.png}
    \caption{An overview of our final model.}
    \label{fig:model}
\end{figure}



\subsection{Verb Classification}
\label{sec:verb}
The verb classification is a rudiment motion-related video understanding task,
where given a video clip, 
our model is required to classify the verb for the most salient event
in the clip.
We follow the standard in VidSitu:
non-visual and fine-grained verb-senses are manually discarded 
and there are in total 	2154 verb-senses for classification.
As our visual event embedding provides a more overall understanding about an event
and what's happening in the video,
we believe our model could achieve higher performance.

The model architecture is simple:
We directly feed the visual event embedding into a classification layer
and train our model with a cross-entropy loss.
The classification layer consists of two linear transformations 
with a ReLU activation layer in between.

\[
p = W_2 \ \mathrm{ReLU}(W_1 e_{\text{event}} + b_1) + b_2
\]

We set the bottleneck dimension to $\frac{F_1+F_2}2$.
That is $W_1: \mathbb{R}^{F_1+F_2} \to \mathbb{R}^{(F_1+F_2)/2}$
and $W_2: \mathbb{R}^{(F_1+F_2)/2} \to \mathbb{R}^{|V|}$,
where $V$ is the set of all candidate verb-senses.

\subsection{Argument Role Prediction}
\label{sec:argument}
In order to test the fidelity of argument information contained in the visual event embedding,
given verbs for every 2-second clip, 
our model is required to predict the arguments of the event.
We still follow the baseline seq-to-seq model from \cite{sadhu2021visual}, 
except that $e_{\text{event}}$ are used as the input for transformer encoder.

To clarify, we freeze the model trained for verb classification task
and get $e_{\text{event}}, ome_{\text{object}}, e_{\text{inter.}}$ for every clip in the first step.
After that,
in order to combine the event embedding with object and interaction embeddings,
for video clip $i\in\{1, 2, 3, 4, 5\}$, 
we define:

\[
e_i = \left[e_{\text{event}}, \frac 1{|\mathcal{O}_i|+1} \left( \sum_{o \in \mathcal{O}_i} ome_o + e_{\text{inter.}}\right)\right],
\]

\noindent where $\mathcal{O}_i$ is the set of objects in event $i$ with top-$K$ confidence.
Since a video is split into 5 clips,
to get a joint understanding about the story,
$e_1, e_2, e_3, e_4, e_5$ are passed into a Transformer \cite{vaswani2017attention} encoder,
getting a contextualized event embedding sequence $e'_1, e'_2, e'_3, e'_4, e'_5$.
For every single clip,
we feed the contextualized event embedding $e'_i$ 
into a TransFormer decoder to generate a sequence of arguments and roles.
To illustrate, in the ``bull-knock-man'' example,
the input of decoder is ``knock [Arg0] gray bull [Arg1] man in gray hoodie ...''
and the target output is ``[Arg0] gray bull [Arg1] man in gray hoodie ...''.
The overall model for argument role prediction is shown in figure \ref{fig:arg_model}.

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.6]{AAAI 2023/image/argument.png}
    \caption{An overview of our model for argument role prediction.}
    \label{fig:arg_model}
\end{figure*}

Because the object and argument information are encoded into the visual event embedding,
we believe that it is easier to decode the correct argument for the model.

%\subsection{Event Contrastive Loss}

%When it comes to injecting the textual event knowledge into a visual model,
%we propose the event contrastive loss to align visual and textual event information.
%To elaborate,
%on the visual side,
%we've obtained the OME for every object in the video,
%while with the help of modern pre-trained language model,
%we can extract an event-entity graph from the textual labels.
%Based on the assumption that the visual event is the sum of all its arguments' states changing,
%the event contrastive loss is designed 
%to align the sum of all visual objects' OME 
%and the sum of all textual arguments' embedding,
%as shown in figure \ref{fig:event_contrastive}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.25]{AAAI 2023/image/event_contrastive.png}
%    \caption{Computation of event contrastive loss.}
%    \label{fig:event_contrastive}
%\end{figure}

%The negative example for event contrastive loss
%would be other textual events from the same training batch,
%which means if the visual and textual embedding describe the same event,
%we make them close to each other.


==> 3exp.tex <==










\section{Experiments}

% \heng{need to add some qualitative analysis with good examples}

\subsection{Dataset}

We evaluate our model on VidSitu \cite{sadhu2021visual}, the public video dataset providing extensive verb and argument structure annotations for more than 130k video clips. Each video clip is approximately two seconds in length with 10 verbs annotated in the evaluation split, and one verb annotated in the training split. There are 2154 verb-senses defined in the event ontology, and each verb has at least 3 semantic roles. 
% which is a novel and complete video situation recognition dataset 
% containing 29K 10-second videos.
% The videos are clipped into 2-second segments and 
% each segment is annotated with its most salient event,
% including a verb and semantic-roles.
% As the video clips are trimmed from movies,
% most of the events are visual related.
% We also aim to show the robustness of the model since the dataset presents complex visual scenes drawn from films covering a wide range of scenarios. 
Table~\ref{tab:statistics} shows the dataset statistics. 
Note that the testing split is hidden and preserved for a leaderboard\footnote{\url{https://leaderboard.allenai.org/vidsitu-verbs/submissions/public}}. 

\begin{table}[h]
\centering
\begin{tabular}{l |c c c c}
\toprule
 & Train & Valid & Test-Verb & Test-Role  \\
\midrule
\# Clip & 118,130 & 6,630 & 6,765 & 7,990  \\
\# Verb  & 118,130 & 66,300 & 67,650 & 79,900 \\
\# Role  & 118,130 & 19,890 & 20,295 & 23,970 \\
\bottomrule
\end{tabular}
\caption{Data statistics. 
% \manling{object statistics?} 
% \manling{only one role for each verb in training set?}
}
\label{tab:statistics}
\end{table}

% Besides a verb and its semantic-roles,
% VidSitu also provides annotations indicating 
% whether arguments involved in multiple events 
% are the same or not,
% which is used for co-referencing.
% Moreover, VidSitu gives links between the events within a same video,
% indicating the relations between different events in a video.
% The model with event knowledge for co-referencing and event relation prediction tasks
% is left for future work,
% and we don't discuss these two tasks in this paper.

% Generally speaking, 
% we implement our model for two tasks on the VidSitu dataset:
% Verb classification and argument prediction given verbs.

% All of our experiments focus on the VidSitu dataset.




\begin{table*}
\setlength\tabcolsep{4pt}
\setlength\extrarowheight{1pt}
\centering
\begin{tabular}{l c|c c c c|c c c c}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Kinetics} & \multicolumn{4}{c|}{Val} & \multicolumn{4}{c}{Test} \\
& & Acc@1 & Acc@5 & Rec@5 & F\textsubscript{1}@5 & Acc@1 & Acc@5 & Rec@5 & F\textsubscript{1}@5 \\
\midrule
TimeSformer & \cmark & 45.91 & 79.97 & 23.61 & 18.23 & - & - & - & - \\
\midrule
I3D$^\dagger$ & \xmark & 30.17 & 66.83 & 4.88 & 4.56 & 31.43 & 67.70 & 5.02 & 4.67 \\
SlowFast$^\dagger$ & \xmark & 32.64 & 69.22 & 6.11 & 5.61 &33.94 & 70.54 & 6.56 & 6.00 \\
I3D$^\dagger$ & \cmark & 29.65 & 60.77 & 18.21 & 14.01 & 29.87 & 59.10 & 19.54 & 14.68 \\
SlowFast$^\dagger$ & \cmark & 46.79 & 75.90 & 23.38 & 17.87 & 46.37 & 75.28 & 25.78 & 19.20 \\

% \midrule
\hline\rowcolor{gray!20}
%SlowFast & \xmark & 33.56 & 72.47 & 6.44 & 5.91 &  &  &  &  \\
%SlowFast & \cmark & 49.77 & 80.86 & 27.20 & 20.35 & & & & \\
\rowcolor{gray!20}
Ours (OSE-pixel\ \ \ \ \ \ \ \ \ \ +\ OME\ ) & \cmark & 52.75 & 83.88 & 28.44 & 21.24 & 52.14 & \textbf{83.84} & 30.66 & 22.45\\
\rowcolor{gray!20}
Ours (OSE-pixel/disp \ +\ OME\ ) & \cmark & 53.32 & \textbf{84.00} & 28.61 & 21.34 & 51.88& 83.55 & \textbf{30.83} & \textbf{22.52}\\
\rowcolor{gray!20}
Ours (OSE-pixel/disp \ +\ OME\ +\ OIE\ ) & \cmark & \textbf{53.36} & 83.94 & \textbf{28.72} & \textbf{21.40} & \textbf{52.39} & 83.47 & 30.74 & 22.47\\
% \bottomrule
\Xhline{2\arrayrulewidth}
\end{tabular}

\caption{\textbf{Results (\%) on verb classification.} ``Kinetics'' denotes whether the model is pre-trained on Kinetics-400 dataset. 
``OSE-pixel'' represents Object State Embedding with in-bounding-box features, and ``OSE-pixel/disp'' adds displacement capturing. ``OME'' stands for Object Motion-aware Embedding and ``OIE'' for Object Interaction Embedding. 
% ``Feat. Ave.'' means we add grid feature average into OSE, ``Disp.'' means we add coordinates into OSE, 
% and ``Int.'' means we add OIE into our model.
Results with $\dagger$ is the performance reported in VidSitu paper \cite{sadhu2021visual}. 
% \xudong{where do we plan to add timesformer results? I think we really need one recent strong video model for comparison.}
}
\label{tab:verb_class}

\end{table*}











\begin{table*}[h]
\centering
\setlength\tabcolsep{6pt}
\setlength\extrarowheight{1pt}
\begin{tabular}{m{5.5cm} |m{2.5cm}<{\centering} | m{2.5cm}<{\centering} | m{2.5cm}<{\centering} | m{2.5cm}<{\centering}}
\toprule
% \multirow{2}{*}{Model} & \multicolumn{4}{c}{Val} \\
\multirow{2}{*}{Model} & CIDEr & CIDEr-Verb & CIDEr-Arg & ROUGE-L  \\
& Avg \quad Std & Avg \quad Std & Avg \quad Std & Avg \quad Std \\
\midrule
\demph{GPT2$^\dagger$} & \demph{34.67} & \demph{42.97} & \demph{34.45} & \demph{40.08} 
\\
\demph{I3D$^\dagger$} & \demph{47.06} & \demph{51.67} & \demph{42.76} & \demph{42.41} 
\\
\demph{SlowFast$^\dagger$} & \demph{45.52} & \demph{55.47} & \demph{42.82} & \demph{42.66} 
\\
% \multirow{2}{*}{SlowFast} 
SlowFast & 44.49 $\pm$2.30 & 51.73 $\pm$2.70 & 40.93 $\pm$2.42  & 40.83 $\pm$1.27 \\
%  & $\pm 2.30$ & $\pm 2.70$ &  & $\pm 1.27$ \\
% \midrule 
\hline
\rowcolor{gray!20}
Ours (OSE-pixel\ \ \ \ \ \ \ \ \ \ +\ OME\ )  & 47.82 $\pm$2.12 & 54.51 $\pm$3.00 & 44.32 $\pm$2.45 & 40.91 $\pm$1.32 \\
% (Ave.) & $\pm 2.12$  & $\pm 3.00$ & $\pm 2.45$ & $\pm 1.32$\\
%  \midrule
\rowcolor{gray!20}
Ours (OSE-pixel/disp \ +\ OME\ )  & \textbf{48.46 $\pm$1.84} & \textbf{56.04 $\pm$2.12} & \textbf{44.60 $\pm$2.33} & \textbf{41.89 $\pm$1.12} \\
% (Ave. + Disp.) & $\pm 1.84$ & $\pm 2.12$ & $\pm 2.33$ & $\pm 1.12$ \\
% \midrule
\rowcolor{gray!20}
Ours (OSE-pixel/disp \ +\ OME\ +\ OIE\ ) & 47.16 $\pm$1.71 & 53.96 $\pm$1.32 & 42.78 $\pm$2.74 & 40.86 $\pm$2.54 \\
% (Ave. + Disp. + Int.) & $\pm 1.71$ & $\pm 1.32$ & $\pm 2.74$ & $\pm 2.54$ \\
% \bottomrule
\Xhline{2\arrayrulewidth}
\end{tabular}

\caption{\textbf{Results on semantic role prediction.} 
% Feat. is the frozen feature extraction model
% used to pre-process videos. C: micro-averaged CIDEr, C-Vb: macro-averaged CIDEr over all verb-senses,
% C-Ag: macro-averaged CIDEr over all arguments. R-L: ROUGE-L score for completeness.
Results are the average (Avg) over 10 runs with standard deviation (Std) reported. The result with $\dagger$ is the single-run performance reported in VidSitu paper \cite{sadhu2021visual}, which is not a fair comparison due to the high variance of free-form generated argument names, so its color is dimmed.
}
\label{tab:sem_pred}

\end{table*}

% \begin{table}[h]
% \centering
% \begin{tabular}{l |c c c c}
% \toprule
% \multirow{2}{*}{Feat.} & \multicolumn{4}{c}{Val} \\
%  & C & C-Verb & C-Arg & R-L  \\
% \midrule
% SlowFast & 45.52 & 55.47 & 42.82 & 42.66 \\
% \multirow{2}{*}{SlowFast} & 44.49  & 51.73& 40.93  & 40.83 \\
%  & $\pm 2.30$ & $\pm 2.70$ & $\pm 2.42$ & $\pm 1.27$ \\
% \midrule
% SlowFast  & 47.82 & 54.51 & 44.32 & 40.91 \\
% (Ave.) & $\pm 2.12$  & $\pm 3.00$ & $\pm 2.45$ & $\pm 1.32$\\
%  \midrule
% SlowFast  & 48.46& 56.04 & 44.60 & 41.89 \\
% (Ave. + Disp.) & $\pm 1.84$ & $\pm 2.12$ & $\pm 2.33$ & $\pm 1.12$ \\
% \midrule
% SlowFast & 47.16 & 53.96 & 42.78 & 40.86 \\
% (Ave. + Disp. + Int.) & $\pm 1.71$ & $\pm 1.32$ & $\pm 2.74$ & $\pm 2.54$ \\
% \bottomrule
% \end{tabular}

% \caption{\textbf{Semantic role prediction metrics.} Feat. is the frozen feature extraction model
% used to pre-process videos. C: micro-averaged CIDEr, C-Vb: macro-averaged CIDEr over all verb-senses,
% C-Ag: macro-averaged CIDEr over all arguments. R-L: ROUGE-L score for completeness.}
% \label{tab:sem_pred}

% \end{table}








\subsection{Evaluation Metrics}

\noindent
\textbf{Verb Classification}
Since each video clip in validation or test split is annotated with 10 verbs,
% all of which are regarded as ground-truth or relevant element.
We predict top-$K$ verbs and calculate ranking-based metrics including Accuracy@$K$, Recall@$K$ and F\textsubscript{1}@$K$, and set $k=5$ in experiments following~\cite{sadhu2021visual}. Also, we report Accuracy@1 as an indicator of its precision in making predictions.
% The top-$K$ predictions of our model
% are treated as retrieved elements and
% in this way, we can get Acc@$K$, Rec@$K$ and F\textsubscript{1}@$K$.
% For convenience,
% we report Acc@1, Acc@5, Rec@5 and F\textsubscript{1}@5.
% For this task, we basically follows the metric in VidSitu \cite{sadhu2021visual},
% except that we additionally report the F\textsubscript{1}@5 score
% for reference.
% Because of the ambiguity in verbs,
% commonly used metrics such as accuracy and F\textsubscript{1}
% are ill suited as they would penalize correct predictions absent from the ground-truth \cite{sadhu2021visual}.
% Therefore, Rec@5 would be the best metric and other metrics are provided as additional information.

\noindent
\textbf{Semantic Role Prediction}
We follow~\cite{sadhu2021visual} to measure 
% the metrics used in VidSitu: only measuring 
the prediction of \textsc{Arg$_{0}$}, \textsc{Arg$_{1}$}, \textsc{Arg$_{2}$}, \textsc{Arg\textsubscript{Loc}} and \textsc{Arg\textsubscript{Scene}}. Since the argument prediction is free-form generation, for every prediction of a semantic role,
we compute the CIDEr score~\cite{vedantam2015cider} by
treating the model prediction as candidate sentence 
and annotations as ground-truth descriptions.
Micro-averaged CIDEr score is computed over each individual prediction,
while macro-averaged CIDEr score is computed over every verb-sense (CIDEr-Verb) and 
over argument-types (CIDEr-Arg).
Also, 
we compute ROUGE-L \cite{lin2004rouge} for longest common subsequence
to show the completeness of generated arguments.

\subsection{Baselines}
\paragraph{State-of-the-art models}
We compare with the state-of-the-art model in~\cite{sadhu2021visual}, which contains two variants, 
% As no new model has been designed for VidSitu after its publication,
% all of our baselines are borrowed from VidSitu \cite{sadhu2021visual}, 
including I3D~\cite{carreira2017quo} and SlowFast~\cite{feichtenhofer2019slowfast}.
For all baselines, we consider the variant with Non-Local blocks \cite{wang2018non},
which has been proved to be more effective according to VidSitu \cite{sadhu2021visual}. We provide their performance reported in the paper. 

We also include a strong transformer-based video model, TimeSformer~\cite{bertasius2021space} as an extra baseline to comprehensively assess the performance of our model. As it is not officially evaluated on VidSitu, we tried our best to search for a suitable hyper-parameter setting on this dataset. 

For semantic role prediction task, apart from reporting the performance of the state-of-the-art models in~\cite{sadhu2021visual}, we also include a text-only decoder GPT2~\cite{radford2019language} as a reference baseline since arguments are predicted via free-form generation. %following~\cite{sadhu2021visual}. 

Unlike verb classification, semantic role prediction results have large variance between difference runs due to free-form generation of argument names. As a result, instead of only reporting performance of a single run, we perform 10 runs and report the average performance (Avg) as well as the standard deviation (Std), as shown in Table~\ref{tab:sem_pred}. %result over 10 different random seeds.
For fair comparison, we re-run the state-of-the-art model\footnote{\url{https://github.com/TheShadow29/VidSitu}} using the best-performed SlowFast backbone for 10 times, and report its average and the standard deviation, which is comparable to the performance reported in its paper~\cite{sadhu2021visual}. 
We also include the original scores as a reference in Table~\ref{tab:sem_pred} but dim the color to indicate that they are not fair comparison.
Also, we are unable to report the performance on the hidden testing split due to the difficulty of submitting each model 10 times to leaderboard repeatedly, so the average performance is only reported on the validation split.
% we're unable to get the average score on test set.
% Consequently, only validation result is show in table \ref{tab:sem_pred}.
% test the fidelity of argument information contained in the visual event embedding, 
% We found that the results of semantic role prediction is unstable,
% so unlike VidSitu,
% which only reports performance of a single run,
% we give the average result over 10 different random seeds.
% Also, because of the leaderboard mechanism,
% we're unable to get the average score on test set.
% Consequently, only validation result is show in table \ref{tab:sem_pred}.


% For SlowFast model, the grid features are passed through an average pooling layer
% to get $e_{\text{all}}^{\text{slow}}$ and $e_{\text{all}}^{\text{fast}}$.
% After that, $[e_{\text{all}}^{\text{slow}}, e_{\text{all}}^{\text{fast}}]$
% is fed into a classification layer.
% Similarly, for I3D model,
% the extracted feature is directly classified.
% All baselines are trained over all verb-senses with a cross-entropy loss.

% \paragraph{Semantic Role Prediction}
% Following baselines in VidSitu,
% the baselines for semantic-role prediction
% is designed as a seq-to-seq model as well.
% The only difference from our model is that
% in baseline visual event embeddings are replaced
% by SlowFast or I3D extracted feature.

\paragraph{Ablation models} 
We include variants of our model to explore the effectiveness of our proposed mechanisms, including: (1) \textbf{OSE-pixel + OME} by only using Object State Embedding to track \textit{pixel} changes;
%, which is then passed to Object Motion-aware Embedding to gather information across multiple frames;
(2) \textbf{OSE-pixel/disp + OME} by using the full setting of Object State Embedding to track both \textbf{pixel} changes and \textit{displacements}; %with Object Interaction Embedding removed;
(3) \textbf{OSE-pixel/disp + OME + OIE} by using the full setting of Object State Embedding and adding Object Interaction Embedding as well.

Note that Object Motion-aware Embedding (OME) is not removable since it is a crucial component to connect multiple frames via a state aggregator, so we add additional experiments and discussions by exploring the different alternatives of the aggregator.

\subsection{Implementation Details}

\noindent
\paragraph{Verb Classification}
For verb classification task,
We trained our model for 10 epochs and 
report the model with highest validation F\textsubscript{1}@5 score.
The training took about 20 hour on 4 V100 GPUs,
comparable to the original SlowFast baseline. 
The frame sampling rate and dimensions of grid features are following SlowFast~\cite{feichtenhofer2019slowfast}. We keep $d_c = 128$ in our experiments. 
We set the maximum number of objects as $8$, and rank objects in terms of the detection confidence. 
The learning rate is chosen from $\{10^{-4}, 3 \times 10^{-5}\}$
and the batch size for training is set to 8.
We use the Adam optimizer with $\beta_1 = 0.9$, $\beta_2 = 0.99$ and $\epsilon = 10^{-8}$,
and no learning rate scheduler is applied to our training.
For all pre-trained parameters, we shrink their learning rate by 90\%,
which keeps the generalizability of the pre-trained encoder. 

\noindent
\paragraph{Semantic Role Prediction}
The visual event embedding of every video clip
is frozen after verb classification training.
During the training of semantic role prediction task, we only train the sequence-to-sequence model including the Transformer-based encoder and decoder.
The model is trained for 10 epochs and we report 
the performance with highest validation CIDEr.
The learning rate is fixed to $10^{-4}$
and the batch size is set to 8.
We also use the Adam optimizer with $\beta_1 = 0.9, \beta_2 = 0.99$ and $\epsilon=10^{-8}$.
Meanwhile, no learning rate scheduler is applied to our training.

\subsection{Quantitative Analysis}

\noindent
\textbf{Verb Classification}
% Table \ref{tab:verb_class} shows our results on verb classification.
As shown in Table \ref{tab:verb_class}, 
our model outperforms the state-of-the-art models on the leaderboard hidden testing set by 8.19\% $\sim$ 8.56\% absolute gains on Accuracy@5
and 4.88\% $\sim$ 5.05\% absolute gains on Recall@5. 
% achieving a new state-of-the-art records on VidSitu dataset. 
The overall F\textsubscript{1}@5 performance achieves 3.32\% absolute gains (17.3\% relative gains) on testing set and 3.53\% absolute gains (19.8\% relative gains) on the validation set. It shows the success of using argument state changes to determine events. 

% Comparing between our models,
% the results show concatenating coordinates' positional embedding into object state could also improve the model.


% \paragraph
\noindent
\paragraph{Semantic Role Prediction}
As shown in Table~\ref{tab:sem_pred}, our best performing model typically achieves 4\% absolute gains on CIDEr scores, proving the effectiveness of argument-level state tracking in identifying the role of the argument. Additionally, the standard deviation is reduced, demonstrating the robustness of fine-grained argument tracking in event structure parsing.


% \paragraph
\noindent
\paragraph{Pixel Changes vs Displacements}
Comparison between OSE-pixel and OSE-pixel/disp proves that displacement is important in characterizing object states. It is especially effective in the task of semantic role prediction, showing that tracking the position changes of objects is very important for determining the motion of objects, thus being helpful for detecting semantic roles.

% \paragraph
\noindent
\paragraph{Effect of Object Interaction Embedding (OIE)}
Verb classification performance is generally improved by capturing interactions between objects, since verbs, by their nature, describe the interactions between objects. However, it does not provide much assistance on argument role prediction, which focuses primarily on each individual argument.
%Here we find some examples from VidSitu dataset to support our statement.
%As shown in figure \ref{fig:exp},
%since our model tracks the argument structure changes,
%the information from arguments and their interaction are taken into consideration when classifying the %verb.

\noindent
\paragraph{TimeSFormer Comparison}
Although our model uses a low-performing video encoding backbone SlowFast, the performance is higher on TimeSFormer, demonstrating the effectiveness of our event-aware visual embedding. 
% \xudong{I remember we also had relative improvement based on TimeSformer?}
% \manling{currently we do not have, but we can add later}

%\begin{figure*}[p]
%    \centering
%    \includegraphics[scale=0.55]{AAAI 2023/image/examples.png}
%    \caption{
%        \textbf{Effectiveness of encoding argument structure changes on verb classification task.}
%        Our model takes advantage of argument structure changing.
%        The state-of-the-art model is the baseline SlowFast+NL model released in \cite{sadhu2021visual}.
%    }
%    \label{fig:exp}
%\end{figure*}

% \subsection{Discussions}

\noindent
\paragraph{Effect of Object Number} 
As shown in Table~\ref{tab:objectnum}, 
the number of objects does not significantly affect performance, since the Argument Interaction Encoder calculates the attention across multiple objects and will focus on the objects that may play an important role in event detection. 
\begin{table}[ht]
\centering
\setlength\tabcolsep{8pt}
\begin{tabular}{l |c c c c}
\toprule
  & Acc@1 & Acc@5 & Rec@5 & F\textsubscript{1}@5  \\
\midrule
$O_{\text{max}}=2$ & 53.56	& 83.98	& 28.95	& 21.53 \\
$O_{\text{max}}=4$ & 53.56 &	84.10 &	28.51 &	21.29 \\
$O_{\text{max}}=8$ & 53.35 &	83.94 &	28.72 &	21.40 \\
\bottomrule
\end{tabular}
\caption{Results (\%) of different object numbers on verb classification. 
% \manling{object statistics?} 
% \manling{only one role for each verb in training set?}
}
\end{table}


\noindent
\paragraph{State Aggregator Operation in OME} 
There is little difference in performance between various alternatives of object state aggregators, and average pooling is slightly more efficient, indicating that a few parameters are sufficient to encode changes of the state of an object. 

\begin{table}[h]
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{l |c c c c}
\toprule
  & Acc@1 & Acc@5 & Rec@5 & F\textsubscript{1}@5  \\
\midrule
LSTM & 53.23 &	83.76 &	28.57 &	21.30 \\
Average Pooling & 53.32	& 83.97 &	28.64 &	21.36 \\
% $O_{\text{max}}=8$ & 53.35 &	83.94 &	28.72 &	21.40 \\
\bottomrule
\end{tabular}
\caption{Results (\%) of different state aggregator operators on verb classification. 
% \manling{object statistics?} 
% \manling{only one role for each verb in training set?}
}
\label{tab:objectnum}
\end{table}


\subsection{Qualitative Analysis}

Example results in Figure~\ref{fig:case_study} illustrate the successful use of argument state changes as a way of determining events. More examples and analysis are detailed in Appendix due to space limitation. 

According to the first example, two objects do not undergo much change in position or pixel, so our model is able to predict events corresponding to \textsc{look} and \textsc{talk}. However, the SoTA model fails to learn the correlation between object state changes and events, so it predicts events requiring state changes, such as \textsc{stop}, \textsc{turn} and \textsc{move}.
This example illustrates the reason why tracking changes is important to the detection of events. %and cannot just use one single frame

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{AAAI 2023/image/example.pdf}
    \caption{Result comparison between SoTA and our model. }
    \label{fig:case_study}
\end{figure}

The second example illustrates how interactions contribute to the detection of events. 
A person's lips are moving as evidenced by pixel changes, so event \textsc{talk} or \textsc{chew} is largely relevant.
% \textsc{talk} or \textsc{chew} are largely relevant due to the fact that the person's mouth is moving as indicated by pixel changes. so \textsc{talk} or \textsc{chew} largely relevant.  
However, the event \textsc{chew} normally requires the interaction between two objects (a person and the food). Since food is not a participant and there is no interaction with food, our model correctly predict the event as \textsc{talk}. 
However, SoTA does not take into account fine-grained object-level interaction information, so it fails to predict the correct events but instead prefers \textsc{chew}. %based solely on the state change of a single person object in the visual scene.

The third example demonstrates the important of encoding of pixel changes. 
It is evident from the position changes of the man on the right side of the video scene that he is moving downward, leading SoTA to prediction of \textsc{roll} and \textsc{fall}. However, his pixel changes indicate that his arm is waving emotionally, which is typically observed in \textsc{fighting} rather than \textsc{roll}. 
As a result, even when displacements match the event type, pixel changes remain extremely useful as an indicator of events.
% demonstrating that object state embedding is highly informative when it comes to event detection.
% The state changes are very informative when determining events even when displacement matches.

% It involves multiple objects with frequent changes in the state of each object. 
% Even when displacement matches, the state changes are still very informative in terms of determining events. 
% The position changes of the man on the right shows that he is moving down, but his pixel changes shows that he has his arm waving emotionally, which normally seen in \textsc{fighting} rather than \textsc{roll},  indicating object state embedding is very informative in terms of event detection.

% The following example illustrates how changes along the temporal axis matter in event detection.
% A person's lips are moving as evidenced by pixel changes, so the use of /textsc[talk] or /textsc[chew] is largely relevant.

% \xudong{if we don't have enough time for the heat map visualization or grad-cam, we can probably add a sentence like we will provide more examples and analysis in the supplementary?}
% \manling{added}

==> 4related.tex <==
\section{Related Work}

\noindent
\textbf{Event Extraction.} 
Extracting events from images/videos  \cite{yatskar2016situation, pratt2020grounded,sadhu2021visual}, texts \cite{ji2008refining,wang2019hmeae,liu2020event,LinACL2020}, or multimedia \cite{li2020cross,chen2021joint,wen2021resin,li2022clip} has attracted extensive research efforts. One of the key challenges in event extraction is to model the structural nature \cite{wang2019hmeae,li2020cross} of events and their associated argument roles. For example, in the text domain, \citet{wang2019hmeae} leverages modular networks to model the relationship between entities of different argument roles. However, to the best of our knowledge, we are the first to explicitly model the states of objects/entities and their relationships in the rich spatial-temporal dynamics of videos.

\noindent
\textbf{Video Understanding.} Video understanding generally requires the model to capture salient objects \cite{ikizler2010object,gu2018ava}, their motion \cite{wang2016temporal,carreira2017quo,Shou_2019_CVPR} and their interactions \cite{baradel2018object,gao2021video}. End-to-end models \cite{feichtenhofer2019slowfast,bertasius2021space,lin2020context} have shown their abilities to capture certain key information for classifying action in videos, where action is usually a single verb or a simple verb phrase~\cite{Kinetics}. Video event extraction \cite{sadhu2021visual} is a more complicated task than action recognition as it not only requires the model to understand the verb but also the interactions among multiple possible argument roles. \citet{baradel2018object} proposed to learn a reasoning model based on object features for action recognition. However, we first propose to explicitly model the object state, their changes and the interaction of objects for video event extraction.

% \subsection{Video Neural Networks}

\begin{comment}
\paragraph{2D Convolutional + Seq-to-seq Model} Encouraged by the superior performance of convolutional neural networks such as ResNet \cite{he2016deep} on image recognition task, 
the traditional design of video neural network model follows the paradigm of a 2D convolutional model plus a seq-to-seq model like RNN or LSTM, 
where the convolutional model is used to process the frames and the seq-to-seq model is capable of capturing the temporal features in the video. 
To better exploit the spatiotemporal dynamics in videos, in 2017, 
TS-LSTM \cite{ma2019ts} is proposed by incorporating optical flow of video features into a ResNet + LSTM model for better supervision, 
which achieves a higher performance especially on activity recognition task.

\textbf{3D Convolutional Neural Networks} 
Before the prevalence of deep neural networks, 3D convolutional neural networks \cite{ji20123d}, 
as an alternative approach to process videos, 
has been proposed in 2012. 
However, this 3D convolutional architecture hasn’t achieved the state-of-the-art until 2018 when the two-stream inflated 3D-ConvNet (I3D) \cite{carreira2017quo} is proposed, 
where the author compared the performance of 5 different architectures and discovered the exceptional capability of I3D.

% \begin{figure*}[ht]
% \centering
% \includegraphics[scale=0.4]{AAAI 2023/image/3d_models.png}
% \caption{Video architectures discussed in I3D \cite{carreira2017quo}.}
% \label{fig:3d_models}
% \end{figure*}

The most significant issue in designing the video neural network architecture is how to resolve the asymmetry between space and time. 
Traditional 3D convolutional neural networks treat space and time symmetrically, 
while they are highly heterogenous. 
For example, there are long-term dependency in a video and
human eyes always favor slow motion rather than fast motion. 
Based on this assumption, 
the SlowFast model \cite{feichtenhofer2019slowfast} is proposed to capture slow and fast motion separately,
using two pathways with different temporal frequency and convolution kernel to perceive the patterns of slow and fast motion. 
So far, SlowFast model still achieves state-of-the-art performance on video recognition task.
6  bb b bbb 


% \noindent
\textbf{Video Understanding}
Video understanding, which aims at training models capable of understanding video content,
is a fundamental goal of computer vision.
Since the greatest difference between videos and images is the dynamic information,
since most video understanding tasks are related to action, motion and event.

Many event related video understanding tasks and their datasets have been proposed and published in recent years.
Tasks such as action classification \cite{carreira2017quo}, 
video description \cite{wang2019vatex}, 
question answering \cite{yu2019activitynet} and object grounding \cite{sadhu2020video} are somehow related to events and their arguments, 
but none of them try to directly extract from the video a detailed event structure with its argument. 

In 2021, VidSitu dataset \cite{sadhu2021visual} is proposed for video situation recognition task, 
where the model is required to classify the verb of a visual event, 
predict semantic-roles in the event and also the relation between events. 

\end{comment}

==> 5conclusion.tex <==
\section{Conclusions and Future Work}

In this work, built upon modern 3D convolutional neural networks,
we construct the first event-aware video encoding neural network by tracking arguments visual states, 
% Meanwhile, it is also the first model focusing on the natural connection between video with events.
which enables the model to understand event semantic structures. %, including the verb and the arguments with their semantic roles. 
On both verb classification and semantic role prediction tasks in VidSitu,
our model achieved a new state of the art, 
outperforming state-of-the-art 3D convolutional neural networks. 
The promising future of our event-aware video embedding excites us, 
as it is applicable to a wide range of event-related video tasks, including action classification, video description, etc. 
% We plan to adapt our model to more tasks for further evaluation and it might also be beneficial to track argument states in pre-training stage. Especially, the object state aggregator and  argument interaction encoder
% could also get pre-trained.
In addition to adapting our model to more tasks, we will also work on tracking argument states in pre-training stages.

==> AAAI 2023/2model_bak.tex <==
\section{Methodology}
Our goal is to identify events (verbs) in a video clip, and to fill in the semantic roles of each predicted verb with entities (nouns). Our primary idea is to introduce argument-level information by encoding the state changes of all arguments via Object State Embeddings and Object Motion-aware Embeddings, as well as their interactions through Multi-object Interaction Embeddings (Section~\ref{sec:embedding}). 
Afterwards, all objects are globally contextualized via an Argument Interaction Encoder (Section~\ref{sec:encoder}) to pay attention to objects that might be of relevance to main arguments for verb classification (Section~\ref{sec:verb}) and semantic role prediction (Section~\ref{sec:argument}). 
%Then it is followed by an Argument Interaction Encoder to globally contextualize all objects with attention to objects that might be of relevance to main arguments (Section 3) for verb classification (Section 4) and semantic role prediction (Section 5). 
% In this section, we introduce our method in details. We first give the formal definition of the task, introduce each part of our model, and then demonstrate how to apply our model on two event extractions tasks: verb classification and semantic role prediction.

\begin{comment}
Event extraction from unstructured plain text has become a popular and thoroughly-studied research topic,
while due to the heterogeneity and inferiority of visual features,
video event extraction remains to be a much more challenging task.
In natural language processing domain,
there are explicit event trigger words or verbs indicating the happening of events.
However, when it comes to visual event,
only implicit and subtle motion of objects are related to it.
Considering this status quo,
our model is designed to tackle video event extraction by 
encoding argument state changes,
which perfectly matches the definition of events.

Arguments of an event are represented as objects in a video,
so we model the argument state changes as object state changes,
or object motion.
Consequently, sum of all object motion 
naturally contains all information about the event.

Inspired by this intuition, we propose \textbf{Object State Embedding} to 
capture the object states and 
design \textbf{Object Motion-aware Embedding} (OME) to
characterize the motion of an object.
Furthermore, the OME of different objects are utilized by \textbf{Argument Interaction Encoder} to
produce a visual event embedding, which is an overall description of the event in a video.
\end{comment}

\subsection{Problem Formulation}

% Given a video clip $\mathcal{V}$ that last several seconds, the output is 
Given a video clip $V$, the model is required to output a series of events $\{E_1, E_2, \cdots, E_k\}$ occurring in the video. Each event is represented as a semantic structure 
\begin{equation*}
    E_i = \{v_i, 
    \langle r_i^1, a_i^1 \rangle, 
    \langle r_i^2, a_i^2 \rangle, 
    \cdots, 
    \langle r_i^m, a_i^m \rangle
    \},
\end{equation*}
consisting a verb $v_i$ and multiple arguments $\{\langle r_i^j, a_i^j \rangle\}$ of the event. As defined in the event ontology, each verb $v_i$ is chosen from a pre-defined verb set\footnote{There are 1500 unique verbs defined in the event ontology of the video situation recognition dataset  VidSitu~\cite{sadhu2021visual}.} $\mathcal{V}$, and has a pre-defined set of roles $\mathcal{R}(v_i)$. Here, $r_i^j \in \mathcal{R}(v_i)$ represents the $j$\textsuperscript{th} role of the verb $v_i$, and $a_i^j$ denotes the corresponding argument entity, which an open-word word or phrase. 
% Each verb $v_i$ is chosen from a pre-defined verb set $\mathcal{V}$ in the event ontology.
% All verbs $v_i$ are chosen from a pre-defined verb set $\mathcal{V}$, while argument $A_i^j$ is a word or phrase describing the $j$-th role of the event $E_i$. 
% Take Figure~\ref{img:task} as an example. 
For example, the event detected for the video clip in Figure~\ref{img:task} is \textsc{knock}, and main arguments are $\langle$\textsc{agent}, \textit{gray bull}$\rangle$, 
$\langle$\textsc{target}, \textit{midget in gray hoodie}$\rangle$ 
and 
$\langle$\textsc{scene}, \textit{ground}$\rangle$.



% \subsection{Object State Embedding \& Object Motion-aware Embedding}
% \subsection{Object State and Motion Change Tracking}
\subsection{Object Visual State Tracking}
\label{sec:embedding}
From the perspective of kinematics, the motion of an object can be decomposed into transitional and rotational movements, which correspond to the body shift and the rotation of the object, respectively.
Likewise, we apply this paradigm to videos and decompose the object motion into the \emph{displacement} of the bounding box and the \emph{pixel changes} within that bounding box.
% This paradigm can be applied to videos as well, allowing us to decompose motion into displacement of the bounding box and pixels changes within that bounding box.
As shown in Figure~\ref{fig:man_motion}, the displacement of the \textit{man} shows that he is moving from left to right and from near to far, while the pixel changes indicate that he is changing from standing to lying down. 
The motion of the \textit{man} can be well defined by the displacement of it bounding box and the pixel changes. Therefore, we detect objects in the video and propose object state embedding and object motion-aware embedding to encode the displacement and pixel changes of objects.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.4]{AAAI 2023/image/man_motion.png}
    \caption{Bounding boxes of a man in a video.}
    \label{fig:man_motion}
\end{figure}


\paragraph{Object Detection and Tracking} 
%To describe the displacement of an object's bounding box, we adopt VidVRD~\cite{gao2021video}, a state-of-the-art object tracking method, to generate object tracklets. 
We generate object tracklets using the state-of-the-art object tracking model VidVRD~\cite{gao2021video}. Taking a raw video as input, it outputs a list of object tracklets $\{T_j\}_{j=1}^n$, where $n$ is the number of recognized objects. Each $T_j$ with length (number of frame in which the object appears) $l_j$ is characterized by its time slot $(st_j, ed_j)$ and bounding box coordinates $\{b_{ji}\in \mathbb{R}^4|i=st_j,\dots, ed_j\}$.

\paragraph{Video Encoding Backbone} 
To utilize the superior power of 3D convolutional neural networks and improve computation efficiency,
our object state and motion-aware embedding are built upon the state-of-the-art SlowFast model \cite{feichtenhofer2019slowfast},
which is used as a video encoder to get high-level grid features of raw videos.

The video encoder takes as input slow and fast sampled video frames $v_{\text{slow}}\in \mathbb{R}^{T_1\times W \times H \times 3}, v_{\text{fast}}\in \mathbb{R}^{T_2 \times W \times H \times 3}$
and outputs slow and fast grid features $f_{\text{slow}}\in \mathbb{R}^{T_1\times W' \times H' \times F_1},
f_{\text{fast}} \in \mathbb{R}^{T_2 \times W' \times H' \times F_2}$:
\[
    [f_{\text{slow}}, f_{\text{fast}}] = \mathrm{SlowFast}(v_{\text{slow}}, v_{\text{fast}}),
\]
where $W$ and $H$ are the width and height of raw video frames,
and $W'$ and $H'$ are the width and height of the processed grid features.
Notice that $T_1 < T_2$ and both of them are the number of frames sampled from the video,
while $F_1, F_2$ are the number of channels of slow and fast grid features respectively.


\paragraph{Object State Embedding} Now, we focus on the grid feature $f$.
Given the bounding box of an object in a frame of the raw video, we first calculate the corresponding bounding box in the grid feature space, then we mask all grid features outside the bounding box
and only focus on the location and in-bounding-box grid features.
Following the displacement plus pixel changes paradigm,
the state of the object can be characterized as the coordinates of bounding box 
and the grid features within the bounding box.
Therefore,
as shown in figure \ref{fig:state}, we define the \textbf{object state embedding} as 
the concatenation of in-bounding-box grid feature average and coordinates positional embedding,
which represents the state of the object.
% The remaining part is exactly in-bounding-box pixels with their location,
% which means the masked video represents \emph{displacement} and \emph{pixel changes} of the object.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{AAAI 2023/image/object_state.png}
    \caption{State embedding of the man in the first frame.}
    \label{fig:state}
\end{figure}

Formally speaking, we denote $f_i \in \mathbb{R}^{W'\times H' \times F}$ as the slow or fast
grid feature of frame $i$.
Also, we assume left bottom and right top corners of the bounding box of object $j$ in grid feature space are $(\hat b^{0}_{ji}, \hat b^{1}_{ji})$ and $(\hat b^{2}_{ji}, \hat b^{3}_{ji})$.
Then, the object state embedding would be:

\[
\begin{aligned}
c_{ji} & = W_c\hat b_{ji} \\
p_{ji} & = \frac 1{(\hat b^{2}_{ji}-\hat b^{0}_{ji})(\hat b^{3}_{ji}-\hat b^{1}_{ji})} \sum_{x =\hat b^{0}_{ji}}^{\hat b^{2}_{ji}-1} \sum_{y = \hat b^{1}_{ji}}^{\hat b^{0}_{ji}-1} f_{i,x,y} \\
ose_{ji} & = [p_{ji}, c_{ji}] \\
\end{aligned},
\]

\noindent where $c_{ji} \in \mathbb{R}^{C}$, $p_{ji}\in \mathbb{R}^{F}$ and $ose_{ji} \in \mathbb{R}^{F+C}$ are the coordinate, pixel average and object state embedding.
$W_{c} \in \mathbb{R}^{C \times 4}$ is a positional embedding layer and $C$ is a hyper-parameter.
We keep $C = 128$ in our experiments.


\paragraph{Object Motion-aware Embedding} To track the state changes of an object,
we feed the state embeddings of the object into an \emph{object states aggregator},
which could be any sequential model capable of capturing the differences among state embeddings.
Therefore, the output of the model would be an embedding containing all information about 
the object's motion, which we define as \textbf{object motion-aware embedding}.
This process is shown below in figure \ref{fig:motion_embedding}.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.26]{AAAI 2023/image/motion_embedding.png}
    \caption{Object motion-aware embeddings of the man and bull in the video.}
    \label{fig:motion_embedding}
\end{figure}

To elaborate,
the object motion-aware embedding is defined 
as $ome_j = \mathrm{StateAgg}(ose_j)$, where $ose_j\in \mathbb{R}^{T\times(F+C)}$ is the object state embedding,
and $ome_j \in \mathbb{R}^{F+C}$ is the object motion-aware embedding.
Regarding the object state aggregator,
we tried LSTM \cite{hochreiter1997long} and simple average pooling.
The results support that average pooling is powerful enough.

Since the encoder gives slow and fast grid feature, 
we will get both slow and fast object motion-aware embedding 
$ome_j^{\text{slow}} \in \mathbb{R}^{F_1+C}, ome_j^{\text{fast}}\in \mathbb{R}^{F_2+C}$ respectively.

The overall dimension of OME is shrunk to $\frac{F_1+F_2}{\alpha}$ with a linear layer,
for better alignment in argument interaction encoder.
Here $\alpha$ is a hyper-parameter and we set it to 3.

\paragraph{Object Interaction Embedding}
Except for objects' individual motion,
another great factor we need to consider is the interaction between objects.
That is, OME only focuses on the \emph{intra-bounding-box} changes
while the object interactions are the \emph{inter-bounding-box} changes.
To illustrate,
in the ``bull-knock-man'' event,
only when the model knows that the target of the bull is the man will it give the correct extraction of the event.
Therefore, we propose \textbf{Object Interaction Embedding} (OIE) to capture the interaction changes.

To reveal an overall picture of containing all objects,
we first get the union of all bounding box: $\hat{B}_i = \bigcup_{j \in O_i} \hat{b}_{ji}$,
where $O_i$ is the objects' indices in frame $i$ and $\cup$ computes the union of all bounding boxes.
Following the approach to get OME, 
we also construct interaction states and use an interaction aggregator to calculate the OIE:

\[
\begin{aligned}
c_{i} & = W_c\hat B_{i} \\
p_{i} & = \frac 1{(\hat B^{2}_{i}-\hat B^{0}_{i})(\hat B^{3}_{i}-\hat B^{1}_{i})} \sum_{x =\hat B^{0}_{i}}^{\hat B^{2}_{i}-1} \sum_{y = \hat B^{1}_{i}}^{\hat B^{0}_{i}-1} f_{i,x,y} \\
ie_{i} & = [p_{i}, c_{i}] \\
e_{\text{inter.}} & = \mathrm{InterAgg}(ie) \\
\end{aligned},
\]

\noindent where $e_{\text{inter.}}$ is the Object Interaction Embedding and 
for convenience, $\mathrm{InterAgg}$ uses the same architecture as $\mathrm{StateAgg}$.
Notice that we can also get $e_{\text{inter.}}^{\text{slow}}$ 
and $e_{\text{inter.}}^{\text{fast}}$.
Concatenate them and shrink the dimension, and we'll get $e_{\text{inter.}} \in \mathbb{R}^{\frac{F_1+F_2}{\alpha}}$.


\subsection{Argument Interaction Encoder}
\label{sec:encoder}
In a gesture to incorporate knowledge from OME into our model
and gather all of the motion information of arguments,
we design the argument interaction encoder to capture the interactions between different arguments or objects.
The encoder is a single-layer Transformer \cite{vaswani2017attention} taking as input the whole video, the OME of all objects,
and the interaction embedding.
The output of the encoder is a visual event embedding $e_\text{event}$
which contains all the visual information about the event.
For example, in the ``bull-knock-man'' video, we have
\[
\begin{aligned}
e_{\text{all}}^p & = \frac 1{WH} \sum_{x = 0}^{W} \sum_{y = 0}^H f_{p, i, x, y},\quad  p\in\{\text{slow, fast}\} \\
e_{q} & = [e_q^\text{ slow}, e_q^\text{fast}], \quad q \in \{\text{all, inter}\} \\
ome_j & = [ome_j^\text{slow}, ome_j^\text{fast}], \quad j \in \{\text{bull}, \text{man}\}\\
e_{\text{event}} & = \mathrm{TransformerLayer}([e_{\text{all}}; ome_{\text{man}}; ome_{\text{bull}}; e_{\text{inter.}}]) \\
\end{aligned},
\]
where $e_{\text{all}}\in \mathbb{R}^{F_1+F_2}$ is splitted into $\alpha$ tokens
and $e_{\text{event}} \in \mathbb{R}^{F_1+F_2}$ is the concatenation of first $\alpha$ tokens of the output.

The final model is shown in figure \ref{fig:model}.
The visual event embedding is designed for various tasks
including verb classification, argument prediction and co-referencing.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{AAAI 2023/image/final_model.png}
    \caption{An overview of our final model.}
    \label{fig:model}
\end{figure}



\subsection{Verb Classification}
\label{sec:verb}
The verb classification is a rudiment motion-related video understanding task,
where given a video clip, 
our model is required to classify the verb for the most salient event
in the clip.
We follow the standard in VidSitu:
non-visual and fine-grained verb-senses are manually discarded 
and there are in total 	2154 verb-senses for classification.
As our visual event embedding provides a more overall understanding about an event
and what's happening in the video,
we believe our model could achieve higher performance.

The model architecture is simple:
We directly feed the visual event embedding into a classification layer
and train our model with a cross-entropy loss.
The classification layer consists of two linear transformations 
with a ReLU activation layer in between.

\[
p = W_2 \ \mathrm{ReLU}(W_1 e_{\text{event}} + b_1) + b_2
\]

We set the bottleneck dimension to $\frac{F_1+F_2}2$.
That is $W_1: \mathbb{R}^{F_1+F_2} \to \mathbb{R}^{(F_1+F_2)/2}$
and $W_2: \mathbb{R}^{(F_1+F_2)/2} \to \mathbb{R}^{|V|}$,
where $V$ is the set of all candidate verb-senses.

\subsection{Argument Role Prediction}
\label{sec:argument}
In order to test the fidelity of argument information contained in the visual event embedding,
given verbs for every 2-second clip, 
our model is required to predict the arguments of the event.
We still follow the baseline seq-to-seq model from \cite{sadhu2021visual}, 
except that $e_{\text{event}}$ are used as the input for transformer encoder.

To clarify, we freeze the model trained for verb classification task
and get $e_{\text{event}}, ome_{\text{object}}, e_{\text{inter.}}$ for every clip in the first step.
After that,
in order to combine the event embedding with object and interaction embeddings,
for video clip $i\in\{1, 2, 3, 4, 5\}$, 
we define:

\[
e_i = \left[e_{\text{event}}, \frac 1{|\mathcal{O}_i|+1} \left( \sum_{o \in \mathcal{O}_i} ome_o + e_{\text{inter.}}\right)\right],
\]

\noindent where $\mathcal{O}_i$ is the set of objects in event $i$ with top-$K$ confidence.
Since a video is split into 5 clips,
to get a joint understanding about the story,
$e_1, e_2, e_3, e_4, e_5$ are passed into a Transformer \cite{vaswani2017attention} encoder,
getting a contextualized event embedding sequence $e'_1, e'_2, e'_3, e'_4, e'_5$.
For every single clip,
we feed the contextualized event embedding $e'_i$ 
into a TransFormer decoder to generate a sequence of arguments and roles.
To illustrate, in the ``bull-knock-man'' example,
the input of decoder is ``knock [Arg0] gray bull [Arg1] man in gray hoodie ...''
and the target output is ``[Arg0] gray bull [Arg1] man in gray hoodie ...''.
The overall model for argument role prediction is shown in figure \ref{fig:arg_model}.

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.6]{AAAI 2023/image/argument.png}
    \caption{An overview of our model for argument role prediction.}
    \label{fig:arg_model}
\end{figure*}

Because the object and argument information are encoded into the visual event embedding,
we believe that it is easier to decode the correct argument for the model.

%\subsection{Event Contrastive Loss}

%When it comes to injecting the textual event knowledge into a visual model,
%we propose the event contrastive loss to align visual and textual event information.
%To elaborate,
%on the visual side,
%we've obtained the OME for every object in the video,
%while with the help of modern pre-trained language model,
%we can extract an event-entity graph from the textual labels.
%Based on the assumption that the visual event is the sum of all its arguments' states changing,
%the event contrastive loss is designed 
%to align the sum of all visual objects' OME 
%and the sum of all textual arguments' embedding,
%as shown in figure \ref{fig:event_contrastive}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.25]{AAAI 2023/image/event_contrastive.png}
%    \caption{Computation of event contrastive loss.}
%    \label{fig:event_contrastive}
%\end{figure}

%The negative example for event contrastive loss
%would be other textual events from the same training batch,
%which means if the visual and textual embedding describe the same event,
%we make them close to each other.


==> init.tex <==
\usepackage{times}  % DO NOT CHANGE THIS
\usepackage{helvet}  % DO NOT CHANGE THIS
\usepackage{courier}  % DO NOT CHANGE THIS
\usepackage[hyphens]{url}  % DO NOT CHANGE THIS
\usepackage{graphicx} % DO NOT CHANGE THIS
\urlstyle{rm} % DO NOT CHANGE THIS
\def\UrlFont{\rm}  % DO NOT CHANGE THIS
\usepackage{natbib}  % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\usepackage{caption} % DO NOT CHANGE THIS AND DO NOT ADD ANY OPTIONS TO IT
\frenchspacing  % DO NOT CHANGE THIS
\setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS
\setlength{\pdfpageheight}{11in} % DO NOT CHANGE THIS
%
% These are recommended to typeset algorithms but not required. See the subsubsection on algorithms. Remove them if you don't have algorithms in your paper.
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{booktabs}
\usepackage{multirow}

\usepackage{newfloat}
\usepackage{listings}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}
%
% Keep the \pdfinfo as shown here. There's no need
% for you to add the /Title and /Author tags.
\pdfinfo{
/TemplateVersion (2023.1)
}

% DISALLOWED PACKAGES
% \usepackage{authblk} -- This package is specifically forbidden
% \usepackage{balance} -- This package is specifically forbidden
% \usepackage{color (if used in text)
% \usepackage{CJK} -- This package is specifically forbidden
% \usepackage{float} -- This package is specifically forbidden
% \usepackage{flushend} -- This package is specifically forbidden
% \usepackage{fontenc} -- This package is specifically forbidden
% \usepackage{fullpage} -- This package is specifically forbidden
% \usepackage{geometry} -- This package is specifically forbidden
% \usepackage{grffile} -- This package is specifically forbidden
% \usepackage{hyperref} -- This package is specifically forbidden
% \usepackage{navigator} -- This package is specifically forbidden
% (or any other package that embeds links such as navigator or hyperref)
% \indentfirst} -- This package is specifically forbidden
% \layout} -- This package is specifically forbidden
% \multicol} -- This package is specifically forbidden
% \nameref} -- This package is specifically forbidden
% \usepackage{savetrees} -- This package is specifically forbidden
% \usepackage{setspace} -- This package is specifically forbidden
% \usepackage{stfloats} -- This package is specifically forbidden
% \usepackage{tabu} -- This package is specifically forbidden
% \usepackage{titlesec} -- This package is specifically forbidden
% \usepackage{tocbibind} -- This package is specifically forbidden
% \usepackage{ulem} -- This package is specifically forbidden
% \usepackage{wrapfig} -- This package is specifically forbidden
% DISALLOWED COMMANDS
% \nocopyright -- Your paper will not be published if you use this command
% \addtolength -- This command may not be used
% \balance -- This command may not be used
% \baselinestretch -- Your paper will not be published if you use this command
% \clearpage -- No page breaks of any kind may be used for the final version of your paper
% \columnsep -- This command may not be used
% \newpage -- No page breaks of any kind may be used for the final version of your paper
% \pagebreak -- No page breaks of any kind may be used for the final version of your paperr
% \pagestyle -- This command may not be used
% \tiny -- This is not an acceptable font size.
% \vspace{- -- No negative value may be used in proximity of a caption, figure, table, section, subsection, subsubsection, or reference
% \vskip{- -- No negative value may be used to alter spacing above or below a caption, figure, table, section, subsection, subsubsection, or reference

\setcounter{secnumdepth}{2} %May be changed to 1 or 2 if section numbers are desired.

% The file aaai23.sty is the style file for AAAI Press
% proceedings, working notes, and technical reports.
%

\newcommand{\bs}{\boldsymbol}

\usepackage{xcolor}
\usepackage{colortbl}
\definecolor{demphcolor}{gray}{.5}
\newcommand{\demph}[1]{\textcolor{demphcolor}{#1}}
\newcommand{\gtext}[1]{\textcolor{citecolor}{#1}}
\newcommand{\rtext}[1]{\textcolor{red}{#1}}
\usepackage{makecell}

% \usepackage[usenames,dvipsnames]{color}
\newcommand{\grey}[1]{{\color{gray} #1}}
\newcommand{\red}[1]{{\color{red} #1}}
\definecolor{gold}{rgb}{0.83, 0.69, 0.22}
\usepackage{xparse}
\iftrue  % show comments or not

\NewDocumentCommand{\heng}
{ mO{} }{\textcolor{red}{\textsuperscript{\textit{Heng}}\textsf{\textbf{\small[#1]}}}}
\NewDocumentCommand{\manling}
% { mO{} }{\textcolor{blue}{\textsuperscript{\textit{Manling}}\textsf{\textbf{\small[#1]}}}}
{ mO{} }{}
\NewDocumentCommand{\xudong}
{ mO{} }{\textcolor{cyan}{\textsuperscript{\textit{Xudong}}\textsf{\textbf{\small[#1]}}}}

%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
